Optimally Interpolating between Ex-Ante Fairness and Welfare

For the fundamental problem of allocating a set of resources among individuals with varied preferences, the quality of an allocation relates to the degree of fairness and the collective welfare achieved. Unfortunately, in many resource-allocation settings, it is computationally hard to maximize welfare while achieving fairness goals. In this work, we consider ex-ante notions of fairness; popular examples include the \emph{randomized round-robin algorithm} and \emph{sortition mechanism}. We propose a general framework to systematically study the \emph{interpolation} between fairness and welfare goals in a multi-criteria setting. We develop two efficient algorithms ($\varepsilon-Mix$ and $Simple-Mix$) that achieve different trade-off guarantees with respect to fairness and welfare. $\varepsilon-Mix$ achieves an optimal multi-criteria approximation with respect to fairness and welfare, while $Simple-Mix$ achieves optimality up to a constant factor with zero computational overhead beyond the underlying \emph{welfare-maximizing mechanism} and the \emph{ex-ante fair mechanism}. Our framework makes no assumptions on either of the two underlying mechanisms, other than that the fair mechanism produces a distribution over the set of all allocations. Indeed, if these mechanisms are themselves approximation algorithms, our framework will retain the approximation factor, guaranteeing sensitivity to the quality of the underlying mechanisms, while being \emph{oblivious} to them. We also give an extensive experimental analysis for the aforementioned ex-ante fair mechanisms on real data sets, confirming our theoretical analysis.

==> sections/02.notations-old.tex <==
\section{Notations and Framework}
Consider a non-negative value function $V:\Sol \rightarrow \mathbb{R}^{+}_0$ defined on a solution space $\Sol$. We say that the function $V$ assigns a \emph{value} or \emph{welfare}, $V(i)$ to a solution $i \in \Sol$. 

We will consider probability distribution vectors  $p =\{p_i\}_{i \in \Sol}$ over the solution space. Here $p_i \in [0,1]$ specifies the probability assigned to solution $i \in \Sol$. We write $\Delta:=\{p =\{p_i\}_{i \in \Sol}: p_i \in [0,1], \sum_i p_i=1 \}$ to denote the set of all distributions vectors over the solution space $\Sol$. For $p \in \Delta$, we linearly extend the definition of the value function and write $V(p)=\sum_{i\in \Sol} p_i \cdot V(i)$. That is, $V(p)$ is the expected value of a random variable that takes values in the solution space $\Sol$ with distribution $p$. 
Note that the value function can model important welfare functions like \emph{utilitarian welfare} and \emph{Nash social welfare} for classic resource-allocation settings. 

Given a value function $V$, we say that a welfare-maximizing mechanism $\mcl$ has an approximation factor of $\lambda \in [0,1]$ if it outputs a solution $A \in \Sol$ such that $V(A) \geq \lambda \cdot V(\ou)$, where $V(\ou) = \max_{i \in \Sol} V(i)$ is the optimal value for the given value function.

 We assume that a \emph{fair mechanism} can be expressed as a random variable over the space of all solutions and we call the corresponding distribution vector the \emph{fair prior}, and denote it as $\pf \in \Delta$. Furthermore, we assume that our algorithms access the fair prior via a sampling mechanism, i.e., by drawing samples according to the fair prior. Given a distribution vector $p \in \Delta$ over the space of all solutions and a distribution vector $\pf$ of the fair mechanism, we model the distance between $p$ and $\pf$ using the standard notion of total variation. That is, for a fair prior $\pf$ and an  $\alpha \in [0,1]$, we say that $p \in \Delta$ is $\alpha$-fair if  $$\TV(p,\pf):= \frac{1}{2} \cdot \sum_{i\in \Sol}  |p_i-\pf_i| \leq \alpha$$

  
 Given the characterizations of two mechanisms, one that defines the fair prior and the other that is welfare-maximizing, the problem that we are studying is how to optimally interpolate between the two pivotal goals of achieving fairness and maximizing welfare for allocation problems, in a computationally-efficient manner. We define an instance of \emph{fair-to-welfare interpolation} (FWI) as follows. For a value function $V:\Sol \rightarrow \mathbb{R}^+_0$, a fair prior $\pf$ with a sampling mechanism, and a distance threshold parameter $\alpha >0$, we consider the following constrained maximization problem,
\begin{gather*}
\qquad \max_{p \in \Delta} V(p) \\
\text{such that} \ \TV(p,\pf)\leq \alpha
\end{gather*}
of maximizing welfare while preserving fairness guarantees with respect to the total variation distance. Furthermore, for the above problem, we will write $\po \in \Delta$ to denote the optimal distribution, while $\ou \in \Sol$ to denote an optimal solution to the corresponding (unconstrained) welfare maximization problem, i.e., $\ou := argmax_{i\in \Sol} V(i)$. 
Finally, we also assume a black-box access to a welfare-maximizing mechanism $\mathcal{M}_\lambda$ with an approximation factor of $\lambda \leq 1$, that is, it finds a solution $A \in \Sol$ such that $V(A)\geq \lambda \cdot V(\ou)$. 

For our algorithms, we denote an instance of fair-to-welfare interpolation (FWI) by $\mathcal{I}(V,\pf, \mathcal{M}_\lambda, \alpha)$, where $V : \Sol \rightarrow \mathbb{R}^+_0$ is a (welfare) value function over the solution space $\Sol$, $\pf \in \Delta$ is the ex-ante fair prior accessed via a sampling mechanism, $\mathcal{M}_\lambda$ is a welfare-maximizing mechanism with an approximation factor $\lambda \leq 1$, and $\alpha>0$ is a distance threshold with respect to total variation. Given such an instance of FWI, our goal is to interpolate between fairness and welfare guarantees in a computationally efficient manner.





==> sections/03.algorithm.tex <==
\section{Interpolating Between Fairness and Welfare }
In this section, we develop a computationally-efficient algorithm, called $\emix$ that, for any instance of FWI, essentially achieves an optimal multi-criteria approximation with respect to fairness and welfare with a small number of samples drawn from the given ex-ante fair mechanism. Our main result of this section is stated in Theorem~\ref{thm:emix}.

\begin{theorem}\label{thm:emix}
Consider an instance  $\instance$ of FWI along with an approximation factor $\eps>0$ and let $\px$ be the distribution of the output of Algorithm~\ref{alg:cap}. Then, $\px$ is $\alpha$-fair and obtains the following welfare guarantees
\begin{align*}
V(\px) \geq \lambda \cdot (1-\eps) \cdot V(\po).
\end{align*}
using $O(1/\eps^2)$-many samples drawn from the fair prior. 
\end{theorem}


%are interested in achieving \emph{fairness} while maximizing a given \emph{welfare/value function} over a solution space $\Sol$. For any fair-welfare maximization problem $\instance$, an approximation parameter $\varepsilon>0$, and a \lambda-approximation algorithm we develop a computationally-efficient algorithm called $\emix$ (formally detailed in Algorithm \Cref{alg:cap}). $\emix$ uses a black-box access to a $\lambda$-approximation algorithm and a sample mechanism with distribution  $\pf$ for maximizing the value function. The  distribution of $\emix$  is $\alpha$-fair and attains a welfare approximation factor of $\lambda \cdot (1-\eps)$ to $V(\po)$.

%Our algorithm $\emix$ begins by invoking the $\lambda$-approximation algorithm (as a black-box) for solving the unconstrained maximization problem of optimizing the value function (i.e., without the fairness constraint). Let us denote the output of this algorithm by $A \in \mathcal{S}$. With the solution $A$ at our disposal, the key idea is to cleverly interpolate between $A$ and the fair prior pf such that the final distribution maximizes the value function while being $\alpha$-fair.

 The key idea of our algorithm $\emix$ is to redistribute mass from solutions with low welfare in the support of ex-ante fair prior $\pf$ over to the solution provided by the welfare-maximizing mechanism (with approximation factor $\lambda$). 
 The issue with doing this greedily and explicitly is that it is typically computationally infeasible: the solution space may be exponential in the size of the input and even if this is not considered an obstacle, it is computationally infeasible to exactly determine the probability of a mechanism outputting a given solution.

 Instead, we only access the fair prior distribution $\pf$ by independently drawing samples from it. For a given FWI instance, $\emix$ begins with flipping a coin that returns heads with a probability $\alpha$. If the coin flip comes up heads, then it outputs the solution provided by the welfare-maximizing mechanism $\mcl$. Otherwise, it gathers an ensemble of samples from the sampling mechanism and picks a solution that is among the top $(1-\alpha)$-fraction of the highest-valued solutions. Observe that the above-described scheme is a natural way of mimicking the process of moving mass from the $\alpha$-fraction of the smallest-valued solutions in the fair prior $\pf$ to the solution of $\mcl$, only using the sampling mechanism. However, when we are applying this sampling approach we can not guarantee that these $(1-\alpha)$-fraction of the highest-valued solutions of the ensemble are those in the top $(1-\alpha)$-fraction of the highest-valued solution in the support of $\pf$ as well. However, we show that using $O(\eps^{-2})$ many samples, $\emix$ attains a welfare value that is $(1-\eps)$-close to the optimal, i.e., the value we could have obtained with the explicit knowledge of $\pf$. We now present $\emix$ formally in Algorithm~\ref{alg:cap}.
 %This $\eps$ gap is what introduces the extra factor $-\lambda\eps$, compared to the clean $\lambda$ approximation factor we would have obtained if we knew $\pf$ explicitly.  
% A natural approach to solving this could be first flipping a coin that returns .
{
\begin{algorithm}[ht]
{
\caption{Fairness-to-welfare interpolation ($\emix$)}\label{alg:cap}
 {\bf Input:} An instance $\instance$ of FWI, and an approximation factor $\eps>0$. \\
 {\bf Output:} A solution $i \in \Sol$ drawn according to a distribution $\px \in \Delta$ such that $\TV(\px,\pf) \leq \alpha$ and $V(\px)\geq \lambda \cdot (1-\eps)  \cdot V(\po)$. 
\begin{algorithmic}[1]
\STATE Flip a coin that returns heads with probability $\alpha$.
\IF{the coin flip = heads}
\STATE Run $\mcl$ and denote its output by $A \in \Sol$.
   \RETURN $A$
\ELSE \label{alg:else}
   \STATE{Sample $s:=\left\lceil 8((1-\alpha)\eps^2)^{-1}\log(2/\eps)\right\rceil$ many solutions according to the fair prior $\pf$, and  let $Z_s^{()}$ be the vector consisting of these solutions sorted in decreasing order of value.}
   \STATE{Assign one unit of mass, $w_i=1$ to each entry $i\in [s]$ of $Z_s^{()}$.}
   \STATE{Remove a total of $\alpha s$ mass starting from the last entry of $Z_s^{()}$ and moving upwards. Denote the updated weight vector by $w^{\alpha}$}.
%   \COMMENT {Note that the mass last removed from an entry in $Z_s$ might be fractional.}
   \RETURN  a solution from $Z_s^{()}$ chosen with probability proportional to the weight vector $w^{\alpha}$.
\ENDIF
\end{algorithmic}
}
\end{algorithm}
}

We now give our analysis of $\emix$ proving that it is $\alpha$-fair and achieves the claimed $\lambda(1-\eps)$ approximation factor compared to the optimal $V(\po)$. We will prove Theorem~\ref{thm:emix} using  the following two lemmas. The first lemma proves that $\emix$ is $\alpha$-fair.
\begin{lemma}\label{lem:fair}
For any instance,  $\instance$ of FWI, let $\px$ denote the distribution of Algorithm~\ref{alg:cap}'s output. Then, we have
\begin{align*}
  \TV(\px,\pf) = \frac{1}{2}\sum_{i} |\px_i-\pf_i|\leq \alpha.
 \end{align*}
\end{lemma}
Observe that Lemma~\ref{lem:fair} does not depend on the number of samples that $\emix$ draws from the fair prior, i.e. $\emix$ is always $\alpha$-fair. Our next lemma says that the welfare $V(\px)$ of the output distribution is at least $\lambda(1-\eps)$ times the optimal $V(\po)$.
\begin{lemma}\label{lem:aproxemix}
Consider an instance  $\instance$ of FWI. For any $\eps>0$, let $\px$ be the distribution of the output of Algorithm~\ref{alg:cap} obtained by drawing $O(1/\eps^2)$-many samples from the fair prior $\pf$. Then, we have the following welfare guarantee,
\begin{align*}
V(\px) \geq \lambda \cdot (1-\eps) \cdot V(\po).
\end{align*}
\end{lemma}
Combining Lemmas~\ref{lem:fair} and \ref{lem:aproxemix} yields Theorem~\ref{thm:emix}, and hence we move on to their proofs. 
We begin by introducing some useful notation. Let $z_s$ denote a set  of $s$ solutions i.e. $z_s\in \Sol$. We slightly abuse notation and further also consider $z_s$ as an indicator vector over these solutions, where the entries of $z_s$ are sorted in decreasing order of welfare and the $j$'th entry is referred to as $z_s^{(j)}$. Now, for any $\beta \in (0,1)$, consider the following random mechanism $\ta$. It creates a weight vector $w^\beta\in \mathbb{R}^s$ that is initially uniform. Then it removes a total of $\beta s$ mass iteratively, starting with $i=s$ and continuing towards $i=1$, creating a residual vector $w^\beta$. Given this vector $\ta$ picks a solution in $z_s^{()}$ proportional to the weight of $w^\beta$.  By the above discussion, for any $z_s$ we can write
\begin{align}\label{alg:taprop}
\p(\ta(z_s)=i)=\sum_{j=1}^s  \mathbbm{1}_{z_s^{(j)}=i}w_j^\beta /\left((1-\beta)s\right)
\end{align}
Now let $Z_s$ denote a random vector of length $s$, with i.i.d. solutions drawn according to $\pf$. Further, let $Z_s^{(j)}$ denote the $j$'th order variable of $Z_s$ entries in terms of decreasing order. Observe that for $\beta=\alpha$ and $s$ as stated in Step 6, the mechanism $\taa$ works identically to Steps 6-9 in Algorithm~\ref{alg:cap}. Using this together with Equation~(\ref{alg:taprop}) and that $A \in \Sol$ is $\lambda$-approximate welfare-maximizing solution given by $\mcl$, we can write $\px_i$ as follows
\begin{equation}\label{alg:proppx}
\px_i =  \alpha\mathbbm{1}_{i=A}+\sum_{j=1}^s\e \left[\mathbbm{1}_{Z_s^{(j)}=i}\right]\wa_j /s,
\end{equation}
and its expected value $V(\px)$ as 
\begin{align}\label{alg:valuepx}
V(\px)=\alpha V(A)+\sum_{j=1}^s\e \left[V(Z_s^{(j)})\right]\wa_j /s.
\end{align}

It is perhaps instructive to observe that for $\alpha=0$, this mechanism $\tz(z_s)$ corresponds to drawing one entry in $z_s$ uniformly at random. Combining Equations \ref{alg:taprop} and \ref{alg:proppx}, we can write $\pf_i$ as
\begin{align}\label{alg:proppf}
\pf_i= \sum_{j=1}^s\e\left[\mathbbm{1}_{Z_s^{(j)}=i}\right]/s
\end{align}

With the above notation, we are now ready to give the proof of \Cref{lem:fair} i.e. that $\emix$ is $\alpha$-fair. 

\begin{proof}[Proof of Lemma~\ref{lem:fair}]
We need to show that $\TV(\px,\pf)\leq \alpha$, which by definition is equivalent to showing $\sum_{i\in \Sol} \left|\px_i-\pf_i\right|\leq 2\alpha$. For any $i \in [s]$, using the expression of $\px_i$ and $\pf_i$ in equations~(\ref{alg:proppx}) and (\ref{alg:proppf}) respectively, along with the fact that  $\wa_j\leq w_j$ for any $j \in [s]$ and applying the triangle inequality, we get that the absolute difference between $\px_i$ and $\pf_i$ is
\begin{align*} 
 \left|\px_i-\pf_i\right| \leq \alpha\mathbbm{1}_{i=A}+\sum_{j=1}^s\e \left[\mathbbm{1}_{Z_s^{(j)}=i}\right](w_j-\wa_j) /s.
\end{align*}
Now since $\sum_{i\in \Sol} \mathbbm{1}_{Z_s^{(j)}=i}=1$, we obtain using the linearity of expectations that 
\begin{align*}
   \sum_{i\in\Sol}\sum_{j=1}^s\e \left[\mathbbm{1}_{Z_s^{(j)}=i}\right](w_j-\wa_j) /s 
   %&= \sum_{j=1}^{s}(w_j-\wa_j) /s \\
   &= \alpha
\end{align*}
where the last equality follows using $\sum w_j=s$ and $\sum \wa_j=(1-\alpha)s$. Finally, combining the last two equations and using the fact that $\mathbbm{1}_{i=A}=1$ for $i=A$ and zero otherwise, we get the desired bound of $\sum_{i\in \Sol} \left|\px_i-\pf_i\right|\leq 2\alpha$. This completes our proof. 
\end{proof}

Next, we move on to prove Lemma~\ref{lem:aproxemix} that says $\emix$ achieves an $\lambda(1-\eps)$ approximation ratio compared to $V(\po)$. For this, we  introduce some more notation. Recall that $\po$ is the optimal solution to FWI, that is $\TV(\po,\pf)\leq \alpha$ and $V(\po)$ is maximized. In the following, we describe a characterization for the optimal solution $\po$. Start with $\pf$ and remove $\alpha$ mass from the solutions in the $\text{supp}(\pf)$, beginning with the smallest-valued solution and moving towards solutions with higher value. We write $p^{\alpha,r}$ to denote the residual mass left of $\pf$ after the above procedure. Observe that $\po$ is now obtained from $p^{\alpha,r}$ by adding $\alpha$ mass to entry $\ou$. In this way, $\po$ is $\alpha$-fair and it has added as much mass to the optimal solution i.e. it is indeed the optimal solution to the constrained maximization problem of FWI. Note that $\sum_{i\in\Sol}p^{\alpha,r}_i=1-\alpha$ and hence $p^{\alpha,r}/(1-\alpha)$ is a probability measure on the top $(1-\alpha)$-fraction of solutions in $\pf$ (in terms of welfare). In the following, we will use $\paa$ to denote $p^{\alpha,r}/(1-\alpha)$. Finally, $\po$ can be expressed using $\paa$ as follows
\begin{align}\label{alg:proppo}
\po_i=
\alpha\mathbbm{1}_{i=\ou}+(1-\alpha)\paa_i,
\end{align}
implying that 
\begin{align}\label{alg:valuepo0}
V(\po)=\alpha V(\ou)+(1-\alpha)V(\paa).
\end{align}

Moreover, we write $\paac$ to denote $(\pf-p^{\alpha,r})/\alpha$, i.e. a probability measure over the bottom $\alpha$-fraction of solutions in $\pf$ (in terms of welfare). Note that we may decompose $\pf$ using $\paa$ and $\paac$ in the following way
\begin{align}\label{alg:decompf}
\pf=(1-\alpha)\paa+\alpha\paac.
\end{align}



Using the above machinery, we are now ready to present a lemma that will be crucial in proving our Lemma~\ref{lem:aproxemix} that establishes the welfare guarantees for $\emix$. The following lemma says that the expected welfare of a solution picked between the $1-\alpha$-top solutions of an ensemble of $s=\left\lceil 8((1-\alpha)\eps^2)^{-1}\log(2/\eps)\right\rceil$-many samples from the fair prior is close to the expected welfare of $\paa$.

\begin{lemma}\label{cor:valuepx}
Consider an instance  $\instance$ of FWI  and an approximation factor $\eps>0$. Then, we have
\begin{align*}
 \sum_{j=1}^s\e\left[V(Z_s^{(j)})\right]\wa_j /s\geq(1-\alpha)(1-\eps)V(\paa)
\end{align*}

\end{lemma}
The proof of Lemma~\ref{cor:valuepx} appears in the appendix and we now present the proof of Lemma~\ref{lem:aproxemix} that says $\px$ achieves welfare guarantees with an approximation factor of $(1-\eps)\lambda$ as compared to $\po$. 

\begin{proof}[Proof of Lemma~\ref{lem:aproxemix}]
We need to show that $V(\px)$ is lower bounded by $(1-\eps)\lambda V(\po)$. To begin with, using equation~(\ref{alg:valuepx}) we can express $V(\px)$ as 
\begin{align*}
V(\px)=\alpha V(A)+\sum_{j=1}^s \e \left[V(Z_s^{(j)})\right]\wa_j /s.
\end{align*}
Using Lemma~\ref{cor:valuepx} and since $A$ is the solution provided by $\mcl$ i.e., $V(A)\geq \lambda V(\ou)$,  it follows that 
\begin{align}\label{alg:valuepx1}
V(\px)&\geq\alpha \lambda V(\ou)+(1-\alpha)(1-\eps)V(\paa)\nonumber \\
&\geq (1-\eps)(\alpha \lambda V(\ou)+(1-\alpha)V(\paa)).
\end{align}

Recalling the expression for $V(\po)$ from equation~(\ref{alg:valuepo0}) for comparison.
\begin{align}\label{alg:valuepo1}
V(\po)=\alpha  \cdot V\left(\ou\right)+(1-\alpha)  \cdot V\left(\paa\right).
\end{align}

Now, note that, for $a=\alpha  \cdot V\left(\ou\right) $, $b=\alpha \lambda \cdot V \left(\ou\right) $ and $x=(1-\alpha)V(\paa)$, we have $a\geq b$ and $x\geq0 $. Algebraic manipulations then lead to the fact that we must have $\frac{b+x}{a+x}\geq \frac{b}{a}$. Now combining this fact with equations~(\ref{alg:valuepx1}) and (\ref{alg:valuepo1}), we obtain that $\frac{V(\px)}{V\left(\po\right)}$ is lower bounded by 
\begin{align*}
\frac{(1-\eps)(\alpha \lambda \cdot V \left(\ou\right) +(1-\alpha)V(\paa))}{\alpha  \cdot V\left(\ou\right)+(1-\alpha)V\left(\paa\right)}
\geq (1-\eps)\lambda,
\end{align*}
which concludes the proof. 
\end{proof}
\section{Simple Mixing to achieve Fairness and Welfare guarantees}
In this section, we present a faster and simpler algorithm $\smix$ for the problem of fair-to-welfare interpolation (FWI). We show that  $\smix$ is $\alpha$-fair and achieves welfare guarantees that are optimal up to a constant factor. An important feature of $\smix$ is that it has absolutely no computational overhead.
Additionally, we will present the ancillary individual fairness properties beyond the underlying welfare maximizing allocation and the ex-ante fair mechanism at the end of this section.

 For a given FWI instance, $\smix$ proceeds by flipping a coin that returns head with probability $\alpha$. If the coin comes up heads then the algorithm outputs the solution provided by the welfare-maximizing mechanism $\mcl$ else it outputs the solution drawn from the fair sample mechanism. Note that, this can be interpreted as an interpolation between the $\lambda$-approximation solution with $\alpha$ mass and the fair prior distribution scaled with a factor of $1-\alpha$, see  Algorithm~\ref{alg:2approx} below.
. We will show that $\smix$ is $\alpha$-fair and attains an approximation factor of $\min\{\lambda,\alpha \lambda+(1-\alpha)^2\}$. 
 Unlike the $emix$ algorithm, $\smix$ has no computational overhead an in particular it does not have to evaluate any solution.

\input{code/epsilon_mix.tex}
We now present the main theorem of this section stating that $\smix$ is $\alpha$-fair and obtain an approximation factor of $\min\{\lambda,\alpha \lambda+(1-\alpha)^2\}$ compared to the welfare of $\po$

\begin{theorem} \label{thm:smix}
Consider an instance  $\instance$ of FWI and let $\pa$ be the distribution of the output of Algorithm~\ref{alg:2approx}. Then, $\pa$ is $\alpha$-fair and achieves the following welfare guarantee
\begin{align*}
V(\pa) \geq \min\{\lambda,\alpha \lambda+(1-\alpha)^2\} \cdot V(\po).
\end{align*}
\end{theorem}

\begin{remark} \label{rem:smix-welfare}
    Let us consider the ratio of $\min\{\lambda,\alpha \lambda+(1-\alpha)^2\}/\lambda$ and note that it is minimized at $\lambda=1$, and $\alpha=1/2$, i.e. the ratio is lower bounded by $\min\{1,3/4\}=3/4$. And hence, using Theorem~\ref{thm:smix}, we obtain that $\smix$ always achieves the following performance guarantees
    $$V(\pa) \geq \frac{3}{4} \lambda \cdot V(\po)$$
    of being optimal up to constant factors.
\end{remark}

Before proving Theorem~\ref{thm:smix}, we make a few observations about Algorithm~\ref{alg:2approx}. Recall that it returns the solution $A$ (given by the mechanism $\mcl$) with probability $\alpha$ and for the remaining probability, it returns a solution provided by the sampling mechanism for $\pf$. Therefore, for any $i \in \Sol$ we can express the distribution $\pa$ of $\smix$ as follows
\begin{align}\label{alg:proppa}
\pa_i=
\alpha\mathbbm{1}_{i=A}  +(1-\alpha )\pf_i
\end{align}
and, this implies that the expected welfare $V(\pa)$ achieves by $\smix$ may be expressed as
\begin{align}\label{alg:valuepa1}
V(\pa)=\alpha V(A)+(1-\alpha)V(\pf).
\end{align}
Combining this with the fact that $V(A)\geq \lambda V(\ou)$ we  get the following lower bound on $V(\pa)$ 
\begin{align}\label{alg:valuepa0}
V(\pa)\geq \alpha \lambda V(\ou)+(1-\alpha)V(\pf).
\end{align}

Having the above observations, we are now ready to prove Theorem~\ref{thm:smix}.

\input{tikz/score_means.tex}


\begin{proof}[Proof of Theorem \ref{thm:smix}]
We begin by showing that $\pa$ is $\alpha$-fair, i.e. $ \TV(\pa,\pf)\leq \alpha$. By the definition of total variation distance, it suffices to show that $\sum_{i \in \Sol} \left| \pa_i-\pf_i \right|\leq 2\alpha$. We first notice that equation~(\ref{alg:proppa}) implies that $\pa_A\geq \pf_A$ and $\pa_i\leq \pf_i$ for $i\not=A$ i.e., we have $|\pa_A-\pf_A|=\pa_A-\pf_A$ and for $i\not=A$ $|\pa_A-\pf_A|=\pf_A-\pa_A$. We can therefore write
\begin{align*}
&\ \ \ \sum_{i \in \Sol} \left| \pa_i-\pf_i \right|
=\alpha  +\left(1-\alpha \right)
\cdot\pf_{A}-\pf_{A}\\ +& \sum_{i \in \Sol \setminus \{A\}}\pf_i-\left(1-\alpha \right)\pf_i\leq \alpha +  \sum_{i \in \Sol \setminus \{A\}} \alpha\pf_i\leq2\alpha
\end{align*}
proving that $\pa$ is $\alpha$-fair. 

For proving the welfare guarantees of $\smix$, we will show that the ratio $V(\pa)/V(\po)$ is at least as high as $\min\{\lambda,\alpha \lambda+(1-\alpha)^2\}$. We will split this analysis for the ratio into two cases. In the first case, we consider the scenario when $V(\pf)\geq (1-\alpha )V(\ou)$. Using the lower bound of $V(\pa)$ in equation~(\ref{alg:valuepa0}) and the fact that $V(\ou)\geq V(\po)$ we obtain that $V\left(\pa\right)/V\left(\po\right)$ is lower bounded by
\begin{align*}
&\frac{\alpha \lambda V(\ou)+(1-\alpha )^2V(\ou)}{V\left(\po\right)}\geq \alpha \lambda+(1-\alpha)^2.
\end{align*} 
as desired. Therefore, we move to the second case where $V(\pf)\leq (1-\alpha) V(\ou)$. Recall that by using equation~ (\ref{alg:valuepo0}), we can write $V(\po)=\alpha V(\ou)+(1-\alpha)\paa$. Further recall that equation~(\ref{alg:decompf}) says that we can express $\pf=(1-\alpha)\paa+\alpha\paac$ implying that we have $\paa=(\pf-\alpha\paac)/(1-\alpha)$. Now combining the above, we obtain
\begin{align*}
    V(\po)&=\alpha V(\ou)+V(\pf)-\alpha V(\paac)\\
    &\leq \alpha V(\ou)+V(\pf)
\end{align*}
 Since $V(\pa) \leq \alpha \lambda V(\ou)+(1-\alpha)V(\pf)$, we get that the ratio of $V(\pa)/V(\po)$ is lower bounded by
 \begin{align}\label{alg:analytic}
 \frac{\alpha \lambda \cdot V(\ou)+(1-\alpha )\cdot V(\pf)}{\alpha \cdot V(\ou)+V(\pf)}.
 \end{align}
We will now analyze the above expression as a function of $V(\pf)$ and show that it is lower bounded by $\min\{\lambda,\alpha \lambda+(1-\alpha)^2\}$. Note that this will be sufficient to complete our proof. Hence, we move on to show that the expression in equation~(\ref{alg:analytic}) has the desired lower bound for the case when $V(\pf)\leq (1-\alpha) V(\ou)$. 

To this end, consider the function $h(x)=\frac{\alpha \lambda\cdot V(\ou)+(1-\alpha ) x}{\alpha  \cdot V(\ou)+x}$, and its derivative $h'(x)$, as follows
\begin{align*}
%h'(x)&=\frac{\alpha \lambda \cdot V(\ou)+(1-\alpha)x-(1-\alpha )\left(\alpha \cdot  V(\ou)+x\right)}{\left(\alpha \lambda \cdot V(\ou)+(1-\alpha)x\right)^2}\\
\frac{\alpha (1-\alpha) \cdot V(\ou)-\alpha \lambda \cdot  V(\ou)}{\left(\alpha \cdot V(\ou)+x\right)^2}
\end{align*}
We notice that the function $h(\cdot)$ is increasing for $\lambda\leq(1-\alpha)$ and decreasing otherwise. If $h(\cdot)$ is increasing, then $h(x)\geq h(0)= \lambda$ holds true, otherwise if $h(\cdot)$ is decreasing, we have 
$h(x)\geq h((1-\alpha )V(\ou))=\alpha \lambda+(1-\alpha)^2 $ for $x\leq (1-\alpha)  V(\ou)$. This completes our proof and the stated claim holds true.
\end{proof}

\begin{remark}
    The welfare guarantees of \texorpdfstring{\smix}{Lg} are tight. We will give an instance and analysis in the appendix.
\end{remark}



\subsection{Additional Fairness Properties of \texorpdfstring{$\smix$}{Lg}}\label{sec:smix-ind}
For any instance $\instance$ of FWI, the distribution $\pa$ of the output of our algorithm $\smix$ has the following additional property: for any solution $i \in \Sol$ that is in the support of the fair prior $\pf$, i.e., $\pf_i>0$, $i$ is also in the support of $\pa$. This is also the case for $\emix$. However $\smix$ actually, also has the following stronger property that
\begin{align} \label{eq:ind-fair}
\pa_i \geq (1-\alpha) \cdot \pf_i
\end{align}for every solution $i \in \Sol$, with equality for $i\not=A$. 
This follows from the fact that $\smix$ outputs a sample drawn from the fair prior with probability $1-\alpha$. Therefore, in addition to being $\alpha$-fair, $\smix$ preserves the support of the given fair prior as well, hence providing \emph{individual fairness} guarantees. 

Now consider a setting where our FWI framework models the classic problem of allocating a set $[m]$ of $m$ indivisible items to a set $[n]$ of $n$ agents. We say an allocation is an $n$-partition of items into $n$ bundles, one for each agent. Hence, the set of solution space $\Sol$ consists of all possible allocations. An agent $a \in [n]$ has a valuation function $u_a: \Sol \rightarrow \mathbb{R}^+_0$ that defines her utility $u_a(i)$ from an allocation $i \in \Sol$. Note that a distribution vector $p \in \Delta$ is now a random allocation where an allocation $i$ is selected with probability $p_i$. With slight abuse of notation, for any $p \in \Delta$, we say her utility $u_a(p) = \sum_{i \in \Sol} p_i u_a(i)$ is the expected utility she derives from the associated random allocation to the distribution $p$. Finally, the value function $V$ can model social welfare, $V(p)=\sum_{a \in [n]}u_a(p)$ or Nash social welfare $V(i)= (\prod_{a \in [n]} u_a(p))^{1/n}$ of a random allocation associated with $p \in \Delta$. 

Using equation~(\ref{eq:ind-fair}), we can conclude that for any agent $a \in [n]$, her utility in the distribution $\pa$ of $\smix$ is 
\begin{align*}
    u_a(\pa) &= \sum_{i \in \Sol} \pa_i \cdot u_a(i) \\
    & \geq (1- \alpha) \sum_{i \in \Sol} \pf_i \cdot u_a(i) = (1- \alpha) \cdot u_a(\pf)
\end{align*}
at least $(1-\alpha)$ times her utility in the fair prior, hence providing \emph{individual fairness} guarantees in addition to being $\alpha$ to fairness.  

% \section{Comparing the Performance of \texorpdfstring{$\emix$}{Lg} and \texorpdfstring{$\smix$}{Lg}}
% In this section, we show that for any instance of FWI, the expected welfare achieved by $\emix$ is always higher than the expected welfare of $\smix$, that is, $$V(\px) \geq V(\pa)$$

% To begin with, recall that we used $Z_s^{(j)}$ to denote the $j$'th order variable in terms of welfare for $s$-many i.i.d. samples from $\pf$. Using the expression for $\pf$ in terms of $Z_s^{(j)}$, as stated in equation~(\ref{alg:proppf}), we have $V(\pf)= \sum_{j=1}^s\e [V(Z_s^{(j)})]/s$. Combining this with equation~(\ref{alg:valuepa1}) which states that the expected welfare of $\smix$ is $V(\pa)=\alpha V(A)+(1-\alpha)V(\pf)$ we obtain
% $$V(\pa)=\alpha V(A)+(1-\alpha)\sum_{j=1}^s\e [V(Z_s^{(j)})]/s$$
% Therefore, using the expression for the expected welfare of $\emix$, stated in equation~(\ref{alg:valuepx}), we know that proving $V(\px)\geq V(\pa)$ is equivalent to showing that 
% \begin{align} \label{eq:weighted-sum}
%   \frac{\sum_{j=1}^s\e [V(Z_s^{(j)})]\wa_j}{(1-\alpha)s}\geq \frac{\sum_{j=1}^s\e [V(Z_s^{(j)})]}{s}  
% \end{align}
% Now, recall that $\wa$ is an $s$-long vector created from an all one's vector and then removing $\alpha s$ mass starting from the last entry and continuing down towards $1$. Therefore, for every $l \in [s]$, we have $\sum_{j=1}^l\wa_j /((1-\alpha)s)\geq \sum_{j=1}^l 1/s$. Furthermore, due to the ordering of the vector $Z_s^{()}$, we have  $\e[V(Z_s^{(j)})]\geq \e[V(Z_s^{(i)})]\geq 0$ for $j\geq i$. Finally, using the Karamata's inequality \cite{} obtain the desired inequality~(\ref{eq:weighted-sum}). Note that, it essentially implies that a weighted sum of order variables is largest if we push the most mass to the largest variables.



==> sections/04.experiments.tex <==
% \newpage
\section{Experiments}

We complement our theoretical analysis with an extensive practical evaluation.  
$\emix$ should theoretically produce better welfare than $\smix$. Nevertheless, the simplicity of $\smix$, as well as its ancillary individual fairness property begs the question of whether the theoretical performance gap between the two algorithms also exists in practice, or whether $\smix$ is the preferable algorithm.
We conduct an experimental study on two main scenarios: \emph{assignments} and \emph{sortition}. Both have natural ex-ante fair priors and represent practical use cases of our framework.

Due to space restrictions, we refer to the appendix for a detailed description of the experiments. We considered FWI instances both reflecting the ex-ante fair mechanism randomized round-robin (RRR) and sortition. 

For RRR, we considered the problem of matching papers to reviewers using the AAMAS  data set \cite{PrefLib_AAMAS}. Welfare is measured in terms of average reviewer preference for their assigned papers. 
Specifically, we model these problems as weighted $B$-matching in a bipartite graph with one side of the bipartition corresponding to reviewers and the other side corresponding to papers. 
RRR initially samples a random permutation. The reviewers then choose their papers greedy from the top of the available preference list according to the order of the permutation. The selection is repeated in a round-robin fashion until every paper has sufficiently many reviewers.

For sortition, we used the Adults data set \cite{UCI_adult} and following the line of work by \cite{ebadiansortition}, we modeled welfare as voter representation in the generated committee of size $k$. Each individual is viewed as a point in Euclidean space. Representation is modeled as the (squared Euclidean) distance between an individual and its closest representative. The value of a committee of size $k$ is the likelihood of a mixture model of $k$ Gaussians each with an identity covariance matrix centered around the points associated with members of the selected committee. The sortition mechanism starts by selecting an initial committee such that the likelihood is maximized, followed by  replacing some committee members with randomly selected individuals.

Overall, it is  possible to generate a (synthetic) instance where there is a detectable gap between $\emix$ and $\smix$. For real-world instances, this gap typically vanishes, see Figure \ref{fig:means}.
Thus, we conclude that the $\smix$ algorithm, due to its simplicity, speed, and ancillary fairness property is, at least empirically, the algorithm to use.


% \subsubsection{Implementation Details}
%  We run experiments on a 14-core Intel Core i9 10940X machine @3.3GHz with 256GB RAM in 3.8 python \footnote{\UrlFont{\href{anonymous. link}{anonymous code link}}}.
 
% \subsubsection{Parameter Setting}
% We set $\epsilon = 0.1$. $N_{adv}$ and $ N_{wait}$ represented numbers on the advantage side and the waiting side in the bipartite graph separately. For the AAMAS bidding dataset, the number of reviewers is smaller than the number of papers. We set each paper should get three reviewers, therefore, the paper each reviewer could get is $\lceil 3 \cdot \frac{N_{wait}}{N_{adv}}\rceil$. The weight of the reviewer's preference is set as 0 if they have no response or choose "no", set as 0.5 when they choose "maybe", and set to 1 if they selected "yes". 

% To produce a convergence result, $\smix$ needs fewer rounds than $\emix$. We set repeating rounds as 300 for $\smix$ and 150 for $\emix$ in all of datasets.

% {\Huge Template}

% \begin{itemize}
%     \item What are our hypothesis? How do we intend to explore these questions? Give an overview.
%     \item Datasets. Only describe what the data sets consist of, where we got them from and how we prepared the data. You should not yet describe how to analyze them. Wenyue, I believe we got a distance metric for the sortition data. That should be described in this section.
%     \item Mechanisms. Describe the mechanisms here. What is the fair prior, what is the welfare maximizing mechanism.
%     \item Implementation and Analysis Details. Running time is not really a concern, so I wouldn't mention hardware. 
%     But, for example, how did we implement the algorithms? One can for example say that we empirically use XXX samples for eps-Mixing. Did we vary the samples? If yes, mention how many different ranges we took. How are we intending to score a run? Are we aggregating means, medians, something else over YYY many independent runs? Are we reporting SD, variance, etc? 
%     \item Results and Interpretation. What did we see? How do we explain these results? Did it confirm our hypothesis? If no, do we have an explanation?
% \end{itemize}




==> sections/06.conclusionandfuturework.tex <==
% \section{Conclusion and future work}
% In this paper we raised the question is it possible to make a natural trade-off between ex-ante fairness and welfare-maximization. We answered this positively with introducing the notion of fair-to-welfare interpolation problems (FWI). Furthermore we developed two "novel" algorithms $\emix$ and $\smix$. Where $\emix$ using $O(1/\eps^2)$-many samples from the sampling mechanism gives an almost optimal solution and $\emix$ using a single sample from the sampling mechanism obtains an optimal approximation factor up to constants. We employed $\emix$ and $\smix$ on real life data. The results here where inline with the analysis saying that $\emix$ should preform better than $\smix$ but not necessarily by much. 

% In the definition of FWI we used the total variance distance define $\alpha$-fairness. However one could also think of other ways of measuring distances between probability distribution. For instance on could use Kullback–Leibler divergence i.e. $\text{KL}(\pf,p)=\sum_{i\in\Sol} \pf_i\log(\pf_i/p_i)\leq \gamma$. Using the Kullback-Leibler divergence would force $p$ to be such that no $i$ in the support of $\pf$ was set to less than $\pf_i exp(p_i/\pf_i)>0$. This gives an $\gamma$-fair distribution the nice interpretation as always having a probability of picking an fair solution (solutions in support of $\pf$). We notice that $\smix$ with $1-\alpha=\exp(-\gamma)$ would be $\gamma$-fair, where as the case for $\emix$ is not straight forward.  


==> sections/old_alg.tex <==

\section{Interpolating Between Fairness and Welfare}
In this section, we are interested in achieving \emph{fairness} while maximizing a given \emph{welfare/value function} for a system. For any instance, $\mathcal{P}(V,\pf,\alpha)$ of fair-welfare maximization problem and an approximation parameter $\varepsilon>0$, 
we develop a computationally-efficient algorithm called $\emix$ (formally detailed in Algorithm~\ref{alg:cap}), that uses a black-box access to a $g$-approximation algorithm for maximizing the value function and finds a distribution (randomized solution) that is $\alpha$-near to the fair prior $\pf$ while attaining an (expected) value of at least $g \cdot (1-\eps)$ times the optimal value $V(\po)$.
%In this section, we are interested in achieving \emph{fairness} while maximizing a given \emph{welfare/value function} over a solution space $\Sol$. For any fair-welfare maximization problem $\mathcal{P}(V,\pf,\alpha)$, an approximation parameter $\varepsilon>0$, and a g-approximation algorithm 
%we develop a computationally-efficient algorithm called $\emix$ (formally detailed in Algorithm~\ref{alg:cap}). $\emix$ uses a black-box access to the $g$-approximation and $\pf$ for maximizing the value function. The  distribution of $\emix$  is $\alpha$-near to the fair prior $\pf$ and attains a  approximation factor of $g \cdot (1-\eps)$ to $V(\po)$.

Our algorithm begins by invoking the $g$-approximation algorithm (as a black-box) for solving the unconstrained maximization problem of optimizing the value function (i.e., without the fairness constraint). Let us denote the output of this algorithm by $G \in \Sol$. With the solution $G$ at our disposal, the key idea is to cleverly interpolate between $G$ and the fair prior $\pf$ such that the final distribution maximizes the value function while being $\alpha$-distance away from the fair prior with respect to the total variation.


 For an approximation parameter $\eps>0$, our algorithm begins by flipping a coin with an appropriately chosen bias dependent on the distance threshold $\alpha>0$. As a result, it chooses the output $G$ of the $g$-approximation algorithm with probability $\alpha(1-\eps)$, else it samples from the fair prior repeatedly for a certain number of times. Next, it trims the $\alpha(1-\eps)$ fraction of the smallest-valued samples and picks any one of the remaining sample solutions. Intuitively, it can be interpreted as removing a mass of $\alpha(1-\eps)$ from the smallest-valued samples of the fair prior and adding it to  the one that has a guaranteed $g$-approximation to the optimal welfare value. We begin with the formal description of $\emix$ in Algorithm~\ref{alg:cap} below.

%m The main idea of $\emix$ is to redistribute mass from solutions with low welfare in the support of $\pf$ over to the solution provided by the g-approximation algorithm. If we knew $\pf$ we would do this by moving $\alpha$ mass from the solution with the lowest welfare of $\pf$ to solution of the g-approximation algorithm. However we only have access $\pf$ via the sampling mechanism. Thus the challenges is to utilize the information about $\pf$ that the sampling mechanism provides. A natural approch to solve the above would here be to first flip a coin which comes up heads with probabililty $\alpha$. Now if the coin flip is heads return the solution provided by the g-approximation algorithm. Else gather an ensample of sample from the sampling mechanism and pick between the top $1-\alpha$ best solutions. The above is mimicinc moving mass from the $\alpha$ smallest valued solution in $\pf$ to the solution of the g-approximation algorith. However when we are doing this in a sampling approch we can not gaurantee with high propabililty that the $1-\alpha$ fraction of highest valued solutions of the ensample are those of the highest valued $1-\alpha$ fraction of the support of $\pf$. We resolve this in $\emix$ by only removing an $\alpha(1-\eps)$ fraction  $\emix$ solve this challenges in the following way $\alpha(1-\eps)$ picking the g-approximation algorithm, or  by using $\Theta(g^{-1}\eps^{-2}$


%where $V(i) \in \mathbb{R}^{+}_0$ denotes the value of a candidate solution $i \in \Sol$
%\subsection{Epsilon precision mixing}

{
\begin{algorithm}[ht]
{
\caption{Fairness along-with welfare maximization ($\emix$)}\label{alg:cap}
 {\bf Input:} An instance $\mathcal{P}(V,\pf,\alpha)$ of the fair-welfare maximization problem, a sampling mechanism for the fair prior $\pf$, a distance threshold $\alpha>0$, an approximation parameter $\eps>0$, and a black-box access to a $g$-approximation algorithm for maximizing the value function $V$. \\
 {\bf Output:} A solution $i \in \Sol$ drawn according to a distribution $\px \in \Delta$ such that $V(\px)\geq g \cdot (1-\eps)  \cdot V(\po)$ and $\TV(\px,\pf) \leq \alpha$.
\begin{algorithmic}[1]
\STATE Run a $g$-approximation algorithm for maximizing the value function $V$, and denote its output by $G \in \Sol$.
\STATE Flip a coin that returns heads with probability $\beta=\alpha(1-\eps)$.
\IF{the coin flip = heads}
   \RETURN $G$
\ELSE %\left\lceil2(\alpha \eps^2)^{-1}\log\left(\frac{K\beta}{\alpha \cdot \eps}\right)\right\rceil
   \STATE{Sample $s:=\left\lceil2\left(\alpha \eps^2\right)^{-1} \log \left(\frac{K\left(1-\eps\right)}{\eps}\right)\right\rceil$ many solutions according to the fair prior $\pf$, and denote them by a vector $Z_s$ of length $s$. Here, $K := \max_{i \in \Sol} V(i)$. }
   \STATE{Assign one unit of mass, $w_i=1$ to each entry $i\in [s]$ in $Z_s$.}
   \STATE{Remove a total of $\beta \cdot s$ mass from the entries of $Z_s$ starting with the one having the smallest welfare value and continuing upwards. For $i \in [s]$, denote the updated mass of the $i$th entry of $Z_s$ to be $w^r_i$.} \\
   \COMMENT {Note that the mass last removed from an entry in $Z_s$ might be fractional.}
   
   %Move all this $\beta s$ mass to the entry corresponding to $S_G$.}
\ENDIF
\RETURN a solution chosen from $Z_s$ with probability proportional to the updated mass.
\end{algorithmic}
}
\end{algorithm}
}
%$\beta :=\alpha(1-\eps)$, and  $s:=\left\lceil2(\alpha \eps^2)^{-1}\log\left(\frac{K\beta}{\alpha \cdot \eps}\right)\right\rceil$. 
For an instance $\mathcal{P}(V,\pf,\alpha)$ of the fair-welfare maximization problem and an approximation parameter $\eps>0$, we write  $K := \max_{i \in \Sol} V(i)$ to be the maximum value attained by the welfare value function.
Let $G \in \Sol$ be the $g$-approximate solution found in Step $1$ of Algorithm~\ref{alg:cap}, i.e., we have $$V(G)\geq g \cdot \max_{i \in \Sol} V(i) = g \cdot K$$  For $s$-many samples drawn according to the fair prior $\pf$ in Step $6$, we consider a random vector $Z_s$ of size $s$, whose $i$th entry represents the $i$th sample drawn from $\pf$. We will write $\E$ to denote the support of $s$ samples drawn according to the distribution $\pf$. Now, consider a random mechanism   $Y(\cdot)$, independent of $Z_s$, that outputs an entry of $Z_s$ uniformly at random. We will denote the law of $Y(Z_s)$ by $\pz$. Note that, since $\pz$ is the same as $\pf$ we may just as well work with $\pz$, i.e., we have
\begin{align} \label{eq:tv}
    \TV(\px,\pf)=\TV(\px,\pz)
\end{align}
 Now, consider a random mechanism $T(\cdot)$ that takes the vector $Z_s$ of length $s$ and begins by assigning one unit of mass $w_i=1$ for  $i\in [s]$  to each entry, i.e., we have $\sum_i w_i= s$. For $\beta=\alpha(1-\eps)$, the mechanism then removes a total of $\beta \cdot s$ mass iteratively, starting with the entry having the smallest $V(\cdot)$ value (breaking ties arbitrarily), before continuing to the next entry with smallest value (see Steps $7$ and $8$ of Algorithm~\ref{alg:cap}). Denote the remaining mass by $w_i^r$ for the entry $i \in [s]$. Note that we can write 
 \begin{align} \label{eq:mass}
      \sum_{i \in ]s]} w^r_i=(1-\beta)s
 \end{align}
 Finally, $T(\cdot)$ selects a single entry $i \in [s]$ that is proportional to the  weights $w_i^r$. Let us now define a random variable $X$ which flips a coin that returns heads  with probability $\beta$. If the outcome of this coin flip is heads, then $X$ outputs the solution $G$, else it outputs whatever the random variable $T(Z_s)$ does. We write $\px$ to be the law of $X$, i.e., $\px$ is distribution of the output of Algorithm~\ref{alg:cap}. By the law of total probability, we can write the $i$th coordinate of the output distribution $\px$ as

\begin{align} \label{eq:px}
\px_{i}=\beta \cdot \mathbbm{1}_{G=i}+(1-\beta) \cdot \p\left[T(Z_s)=i\right].
\end{align}

We begin by establishing a useful upper bound on the expected value of the optimal distribution for an instance of fair-welfare maximization problem.
\begin{lemma} \label{lem:opt}
Consider an instance  $\mathcal{P}(V,\pf,\alpha)$ of the fair-welfare maximization problem. Then, we have the following upper bound on the expected value of its optimal distribution $\po$,
    \begin{align}\label{eq:po}
 V\left(\po\right)
 \leq \alpha \cdot V\left(\ou\right)+V\left(\pf\right).
 \end{align}
\end{lemma}

\begin{proof}
    Given an instance  $\mathcal{P}(V,\pf,\alpha)$ of the fair-welfare maximization problem, we begin by constructing its optimal distribution $\po \in \Delta$ with an explicit access to the fair prior $\pf$. Let us write $\ou := \argmax_{i\in \Sol} V(i)$ to denote the solution index with the highest welfare value. The idea is to modify the fair prior by moving a total of $\alpha$ mass to the index $\ou$ by removing it from the index with the smallest welfare value in $\pf$ and continuing upwards (while breaking ties arbitrarily). We will denote $\pr_i \leq p^f_i$ as the amount of mass removed from $\pf_i$ during the above process. Note that, we can write $||\pr||_1=\sum_i \pr_i=\alpha$, 
and hence, 
\begin{align} \label{eq:pr-dist}
    \frac{\pr}{||\pr||_1}=\frac{\pr}{\alpha} \in  \Delta .
\end{align}
Observe that, the above process leads to a solution that satisfies the fairness constraint of being $\alpha$-close to fair prior $\pf$ (with respect to the total variational distance), while putting as much mass as possible onto an index that maximizes $V(\cdot)$ value. Hence, it yields an optimal distribution---we refer to as $\po$---for the given instance. From this construction of $\po$, we obtain
\begin{align}\label{eq:po}
 V\left(\po\right)&=\sum_{i \in \Sol}\po_i \cdot V(i) \nonumber \\
 &=\alpha \cdot V(\ou)+\sum_{i \in \Sol }(\pf_i-\pr_i)V(i)\nonumber\\
 &=\alpha \cdot V\left(\ou\right)+V\left(\pf\right)-\alpha \cdot V\left(\frac{\pr}{\alpha}\right) 
 \end{align}
This completes our proof and establishes the stated claim.
\end{proof}

Next, we prove that the output distribution of Algorithm~\ref{alg:cap} is $\alpha$-away from the given fair prior  
We now begin our analysis by proving the correctness of  in the following lemma.
\begin{lemma}\label{lem:fair}
Consider an instance  $\mathcal{P}(V,\pf,\alpha)$ of the fair-welfare maximization problem and $\px$ be the output distribution of Algorithm~\ref{alg:cap}, where $\px_i=\p\left[X=i\right]$ is the probability  of selecting index~$i \in \Sol$. Then, we have
\begin{align*}
  \TV(\px,\pf) = \frac{1}{2}\sum_{i} |\px_i-\pf_i|\leq \alpha.
 \end{align*}
\end{lemma}

\begin{proof}
To begin with, recall that, in the above discussion, we argued that $\pz$ is the same as $\pf$, and hence, using equations (\ref{eq:tv}) and (\ref{eq:px}), we can write
\begin{align*}
&\sum_{i\in \Sol} \left|\px_i-\pf_i\right|\\
=&\sum_{i\in \Sol} \left|\px_i-\pz_i\right| \\
=&\sum_{i \in \Sol} |\p\left[X=i\right]-\p\left[Y(Z_s)=i\right]|\\
=&\sum_{i\in \Sol} |\beta  \mathbbm{1}_{G=i}+(1-\beta) \p\left[T(Z_s)=i\right]-\p\left[Y(Z_s)=i\right]|
\end{align*}
By the law of total expectation, we further obtain for any $i\in \Sol$
\begin{align*}
\px_i-\pz_i= \sum\limits_{z\in \E}& \p\left[Z_s=z\right] \cdot \Big(\beta  \mathbbm{1}_{G=i}+(1-\beta)  \\ &\cdot \p\left[T(z)=i\right]-\p\left[Y(z)=i\right]\Big) 
\end{align*}
where,  $\E$ denotes the support of $s$ samples drawn according to the distribution $\pf$.
Finally, by repeated applications of the triangle inequality, we obtain
\begin{align}\label{eq:emixtotalcon}
\sum_{i\in \Sol} |\px_i-&\pz_i| 
\leq  \sum_{z\in \E} \p\left[Z_s=z\right] \nonumber
\sum_{i\in S}| \beta \mathbbm{1}_{G=i}\\&+(1-\beta)  \p\left[T(z)=i\right]-\p\left[Y(z)=i\right]|.   \nonumber
\end{align}
Note that if we can bound the following expression $$\sum_{i\in \Sol} | \left(\beta  \mathbbm{1}_{G=i}+(1-\beta)  \p\left[T(z)=i\right]-\p\left[Y(z)=i\right]\right)|,$$ which we will denote $\mathbb{D}$, such that $D \leq2 \beta$ for any $z\in \E$. We will obtain using \cref{eq:emixtotalcon} the following desired bound on the total variational distance between $\px$ and $\pz$, 
\begin{align*}
    2 \TV(\px,\pz) = \sum_{i\in \Sol} \left|\px_i-\pz_i\right|   \leq \mathbb{D} \leq 2 \beta,
\end{align*}
and since $2\beta\leq 2\alpha$, this completes the proof. 

To this end, we fix a sample set $z\in \E$. Recall that, the mechanism $Y(z)$ returns an index $i \in [s]$ with probability $\p\left[Y(z)=i\right]=\frac{\sum_{j=1}^s w_j \cdot \mathbbm{1}_{(z)_j=i}}{s}$, where $(z)_j \in \Sol$ is the $j$th entry of $z$. On the other hand, since $T(z)$ returns a sample from the entries of $z$ proportional to the (updated) weights $w_i^r$ we obtain $\p\left[T(z)=i\right]=\frac{\sum_{j=1}^s w_j^r \cdot \mathbbm{1}_{(z)_j=i}}{(1-\beta)s}$.  Finally, we use triangle,  inequality, that $\mathbbm{1}_{G=i}=1$ for exactly one index,  $w_j^r\leq w_j$, and \cref{eq:mass} to bound the expression $\mathbb{D}$ as follows, 
\begin{align*}
\mathbb{D}&\leq \beta +\sum_{i\in \Sol}  \frac{|\sum_{j=1}^s \left(w_j^r- w_j\right) \cdot \mathbbm{1}_{(z)_j=i}|}{s} %\tag{since $\mathbbm{1}_{G=i}=1$ for exactly one index.}
\\
&=\beta + \sum_{j=1}^s \sum_{i\in \Sol} \frac{ \left( w_j-w_j^r\right)\cdot \mathbbm{1}_{(z)_j=i}}{s} %\tag{since, $w_j^r\leq w_j$ for all $j \in [s]$}
\\
&=\beta + \frac{ \sum_{j=1}^s  w_j   - \sum_{j=1}^s  w^r_j  }{s} 
\\
& =\beta + \frac{s-(1-\beta)s}{s}= 2\beta, %\tag{using equation (\ref{eq:mass})}
\end{align*}
and, hence the stated claim follows.
\end{proof}

Next, we prove a useful lower bound on the expected welfare of the output distribution of $\emix$.
\begin{lemma} \label{lem:pxlower}
Consider an instance  $\mathcal{P}(V,\pf,\alpha)$ of the fair-welfare maximization problem with a $g$-approximation algorithm to maximize the value function. Then, for the output distribution $\px$ of Algorithm~\ref{alg:cap}, we have
    \begin{align*} V(\px) &\geq \beta g \cdot V \left(\ou\right)\\ &+V(\pf)-\beta \cdot \e\left[\sum_{i\in [s]}\frac{(1-w_i^r) \cdot V((Z_s)_i)}{\beta s}\right] 
\end{align*}
where, $Z_s$ is the random vector of length $s$ comprising of $s$-many samples (as computed in Step 6 of Algorithm~\ref{alg:cap}) and $\beta=\alpha (1-\eps)$.
\end{lemma}

\begin{proof}
   Consider an instance   $\mathcal{P}(V,\pf,\alpha)$ of the fair-welfare maximization problem with the output distribution $\px$ of Algorithm~\ref{alg:cap}. Using  equation~(\ref{eq:px}) and the law of total expectation, we have
\begin{align} \label{eq:vpx}
 V\left(\px\right)=\beta \cdot V \left(G\right) +(1-\beta) \cdot \e\left[V\left(T(z)\right)\right]
\end{align}
where $T(Z_s)$ is as described in the discussion above Lemma~\ref{lem:opt}.
For a sample $z = \{(z)_i\}_{i \in [s]} \in \E$, recall that $T(z)$ is sampled proportional to the updated weights $\{w_i^r\}_i$ and hence, we obtain
\begin{align}
(1-\beta) \cdot V\left(T(z)\right)=&\sum_{i=1}^s \frac{V((z)_i) \cdot w_i^r}{s} \nonumber\\
=\sum_{i=1}^s\frac{ V((z)_i)}{s}-&\sum_{i=1}^s \frac{(1-w_i^r) \cdot V((z)_i)}{s} \nonumber\\
=\sum_{i=1}^s\frac{ V((z)_i)}{s}-&\sum_{i\in R}\frac{(1-w_i^r) \cdot V((z)_i)}{s} \label{eq:tz}
 \end{align}
 where $R \subseteq [s]$ denotes the set of indices from where the mechanism $T(\cdot)$ removes non-zero amount of mass, i.e., $R:= \{i \in [s]: w_i^r<1\}$. Also, we have $1-w_i^r=0$ for all $i \not\in R$ and that $|R|=\left\lceil\beta s\right\rceil$ since $T(\cdot)$ removes a total of $\beta\cdot s$ amount of mass from the vector $z$. Using the linearity of expectations, we can using equation~(\ref{eq:tz}) write $(1-&\beta) \cdot\e\left[V\left(T(Z_s)\right)\right]$ as,
\begin{align*}
\sum_{i=1}^s& \frac{\e\left[V(\left({Z_s}\right)_i)\right]}{s}-\e\left[\sum_{i\in R} \frac{(1-w_i^r) \cdot V((Z_s)_i)}{s} \right]\\
&=V(\pf)-\beta \cdot \e\left[\sum_{i\in R} \frac{(1-w_i^r) \cdot V((Z_s)_i)}{\beta s}\right]
\end{align*}
where the last equality follows from the fact that the entries of $Z_s$ (as computed in Step~6 of Algorithm~(\ref{alg:cap})) are independent samples drawn from the prior $\pf$. Plugging the above expression into equation~(\ref{eq:vpx}), we get that 
\begin{align} \label{eq:px-value}
V(\px)&=\beta \cdot V \left(G\right) +V(\pf)\\&-\beta \cdot \e\left[\sum_{i\in R}\frac{(1-w_i^r) \cdot V((Z_s)_i)}{\beta s}\right] \nonumber\\
&\geq \beta g \cdot V \left(\ou\right)  \nonumber+V(\pf)\\
&-\beta \cdot \e\left[\sum_{i\in R}\frac{(1-w_i^r) \cdot V((Z_s)_i)}{\beta s}\right]  \nonumber
\end{align}
where, the last inequality follows from the fact that $V(G) \geq g \cdot V(\ou)$. The stated claim stands proven.

\end{proof}


We are now ready to establish the desired fairness and welfare guarantees attained by Algorithm~\ref{alg:cap} in the following theorem.
\begin{theorem}\label{thm:emix}
Consider an instance  $\mathcal{P}(V,\pf,\alpha)$ of the fair-welfare maximization problem with a $g$-approximation algorithm to maximize the value function. Then, for any $\eps>0$, Algorithm~\ref{alg:cap} requires $s := \left\lceil2\left(\alpha \eps^2\right)^{-1} \log \left(\frac{K\left(1-\eps\right)}{\eps}\right)\right\rceil $ many samples of the fair prior $\pf$ to find a distribution $\px \in \Delta$ that has the following fairness and welfare guarantees.
\begin{align*}
\TV(\px,\pf) \leq \alpha,  \ \text{and} \ V(\px) \geq g \cdot (1-\eps) \cdot V(\po).
\end{align*}
Here, we write $\po$ to denote the optimal distribution of the instance and $K=\max_{i\in \Sol} V(i)$. 
\end{theorem}
\begin{proof}
Given an instance  $\mathcal{P}(V,\pf,\alpha)$ of the fair-welfare maximization problem, let $\px$ denotes the output distribution $\px$ of Algorithm~\ref{alg:cap}. In order to establish the stated approximation guarantee on the expected value on $V(\px)$, we want to argue that for $\beta=\alpha(1-\eps)$,  the ratio $\frac{V(\po)}{V(\px)}$ is not too large. Using Lemmas~\ref{lem:opt} and \ref{lem:pxlower}, we have the following bounds on $V(\po)$ and $V(\px)$.
\begin{align*}
V(\po)&=\alpha \cdot V\left(\ou\right)+V\left(\pf\right)-\alpha \cdot V\left(\frac{\pr}{\alpha}\right) \\
    V(\px)&\geq \beta g \cdot V \left(\ou\right) +V(\pf)\\&-\beta \cdot \e\left[\sum_{i\in R}\frac{(1-w_i^r) \cdot V((Z_s)_i)}{\beta s}\right] 
\end{align*}
We will first prove that the last terms in the above two expressions of $V(\po)$ and $V(\px)$ are close to each other.
%To this end, let us focus at the expression for $V\left(\po\right)$ in equation~(\ref{poeq}), and prove a bound on the last term in the above expression by showing that it is close to $V\left(\frac{\pr}{\alpha}\right)$. In other words, we will show that the expected value of the normalized $V(\cdot)$ values of the entries corresponding to the indices in $R$---the ones in $Z_s$ with the smallest $V(\cdot)$ values---is close to the expected $V(\cdot)$ value of a random variable drawn from the distribution $\frac{\pr}{\alpha}$ (the values in $\text{supp}(\pf)$ with the smallest $V(\cdot)$ values). 
To this end, we describe a sampling producer of $Z_s$ in the following manner. First, consider a coin that returns heads with probability $\alpha$; we will flip such a coin $s$-many times independently.  We denote the corresponding coin flips as $C_1,\ldots,C_s$ and consider the random variable $C=\sum_{i=1}^sC_i$ where $C_i=1$ if and only if the $i$th coin flip returns heads and else $C_i=0$. It is trivial to see that the expectation $\e\left[C\right]=\alpha s$. Now, let us recall the distribution $\frac{\pr}{\alpha}$ as described in Lemma~\ref{lem:opt}, see equation~(\ref{eq:pr-dist}). We sample according to the distribution $\frac{\pr}{\alpha}$ as many times as the number of heads, otherwise, we sample from the distribution $\frac{\pf-\pr}{1-\alpha}$. We call the resulting vector of length $s$ as $Z_s$. Since the random variable $C$ counts the number of heads in the above $s$-many coin flips, it also counts the number of times we sample from the $\frac{\pr}{\alpha}$-distribution. Applying a Chernoff bound on $C$, we obtain, $$\p\left[C-\e\left[C\right]\leq -\alpha s \varepsilon \right]\leq \exp\left(-\alpha s\eps^2/2 \right).$$
The above bound implies that, with a probability of at least $1-\exp\left(-\alpha s\eps^2/2 \right)$, the sample $Z_s$ contains more than $E[C]-\alpha s \varepsilon=\alpha(1-\eps)s=\beta s$ samples from the $\frac{\pr}{\alpha}$-distribution. 

We now consider an outcome of $C=c$ with $c\geq\left\lceil\beta s\right\rceil$. We write $Z_{r_1},\ldots,Z_{r_c}$ to denote the independent samples from the distribution $\frac{\pr}{\alpha}$ in $Z_s$ and $Z_{\bar{r}_1},\ldots,Z_{\bar{r}_{s-c}}$ be the independent samples from the distribution $\frac{\pf-\pr}{1-\alpha}$. Furthermore, we write $(Z_s)^{(1)},\ldots,(Z_s)^{(s)}$ to denote the variables of $Z_s$'s entries ordered in a decreasing manner with respect to their welfare function values. Note that, since $V\left(Z_{r_i}\right)\leq V\left(Z_{\bar{r}_j}\right)$ for all $i,j$, we may assume, without loss of generality, that $(Z_s)^{(j)}={(Z_r)}^{(j)}$ for $j \in [c]$ where ${(Z_r)}^{(j)}$ is the $j$'th order variable ${Z_r}_1,\ldots,{Z_r}_c$ with respect to their welfare function values. Next, we write ${w_{(i)}}^r$ to denote the updated weight (obtained in Step 8 of Algorithm~\ref{alg:cap}) for the $i$'th order variable $(Z_s)^{(i)}$. From the proof of Lemma~\ref{lem:pxlower}, recall that, since $|R|=\left\lceil\beta s\right\rceil$ and a total of $\beta  s$ mass is being removed from the $\left\lceil \beta s \right\rceil$ smallest entries of $Z_s$ at Step 8, for outcomes where $C=c\geq \left\lceil\beta s\right\rceil$ of $C$, we can conclude
\begin{align} \label{eq:bs}
&\sum_{i\in R} \frac{(1-w_{i}^r) \cdot V((Z_s)_i)}{\beta s}\nonumber=\sum_{i=1}^{\left\lceil \beta s \right\rceil} \frac{(1-w_{(i)}^r) \cdot V({(Z_s)}^{(i)})}{\beta s} \nonumber\\
&=\sum_{i=1}^{\left\lceil \beta s \right\rceil} \frac{(1-w_{(i)}^r) \cdot V({(Z_r)}^{(i)})}{\beta s}
\end{align}
Moreover, note that for such outcomes $c$ of $C$ (where $c \geq \left\lceil\beta s\right\rceil$), the following bound holds true for any injective map $\pi :[\left\lceil\beta s\right\rceil]\rightarrow [c]$,
\begin{align} \label{eq:pi}
     &\sum_{i=1}^{\left\lceil \beta s \right\rceil} (1-w^r_{(i)}) \cdot V\left(Z_{r_{\pi(i)}}\right)\nonumber \\\geq &\sum_{i=1}^{\left\lceil \beta s \right\rceil} (1-w^r_{(i)}) \cdot V({(Z_{r})}^{(i)})
\end{align}
Since $\pi$ is an injective map, we know that $Z_{r_{\pi(i)}}$'s are independent random variables drawn from the distribution $\frac{\pr}{\alpha}$. Using equation~(\ref{eq:pi}), we therefore obtain
\begin{align*}
 \beta s  V\left(\frac{\pr}{\alpha}\right) =\e&\left[\sum_{i=1}^{\left\lceil \beta s \right\rceil}  (1-w^r_{(i)})  V(Z_{r_{\pi(i)}})\Big| C\geq \left\lceil\beta s\right\rceil\right]\\
 \geq \e&\left[\sum_{i=1}^{\left\lceil \beta s\right\rceil} (1-w^r_{(i)})  V({(Z_{r})}^{(i)}) \Big| C\geq \left\lceil\beta s\right\rceil \right]
 \end{align*}
Finally, plugging equation~(\ref{eq:bs}) into the above inequality, we obtain
\begin{align*}\label{ordereq}
V\left(\frac{\pr}{\alpha}\right)\geq \e\left[\sum_{i\in R} \frac{(1-w_i^r) \cdot V((Z_s)_i)}{\beta s}\Big| C\geq \left\lceil\beta s\right\rceil \right]
\end{align*}
Now, the law of total expectation implies that we have
\begin{align*}
&\e\left[\sum_{i\in R} \frac{(1-w_i^r) \cdot V((Z_s)_i)}{\beta s}\right] \\
&\leq V\left(\frac{\pr}{\alpha}\right) \left(1-\exp\left(-s\alpha \eps^2/2\right)\right)\\
&+K  \exp\left(-s\alpha \eps^2/2\right)\\
&\leq V\left(\frac{\pr}{\alpha}\right)+K \cdot \exp\left(-s\alpha \eps^2/2\right)\\
&\leq \left(1+\frac{\alpha \eps}{\beta}\right) \cdot V\left(\frac{\pr}{\alpha}\right)
\end{align*}
where, the last inequality follows due to the sample size $s=\left\lceil2\left(\alpha \eps^2\right)^{-1} \log\left( \frac{K\left(1-\eps\right)}{\eps}\right)\right\rceil$. Finally, plugging the above bound back into equation~(\ref{eq:px-value}) and using $\beta=\alpha (1-\eps)$, we obtain
\begin{align}\label{lowerpx}
 &V(\px)\nonumber\geq \beta gV \left(\ou\right) +V(\pf)-\beta\left(1+\frac{\alpha \eps}{\beta}\right) V\left(\frac{\pr}{\alpha}\right)\\
%&=\beta g \cdot V \left(\ou\right) +V(\pf)-\left(\beta+\alpha \eps\right) V\left(\frac{\pr}{\alpha}\right) \nonumber\\
&=\beta g \cdot V \left(\ou\right) +V(\pf)-\alpha  \cdot V\left(\frac{\pr}{\alpha}\right)
\end{align}
Now, note that, for $a=\alpha  \cdot V\left(\ou\right) $, $b=\beta g \cdot V \left(\ou\right) $ and $x=V(\pf)-\alpha  \cdot V\left(\frac{\pr}{\alpha}\right)$, we have $a>b$ and $x>0 $. Simple algebraic manipulations then lead to the fact that we must have $\frac{a+x}{b+x}\leq \frac{a}{b}$. Combining this fact with equations~(\ref{eq:po}) and (\ref{lowerpx}), we finally obtain that $\frac{V\left(\po\right)}{V(\px)}$ is upper bounded by 
\begin{align*}
\frac{\alpha  \cdot V\left(\ou\right)+V\left(\pf\right)-\alpha  \cdot V\left(\frac{\pr}{\alpha}\right)}{\beta g \cdot V \left(\ou\right) +V(\pf)-\alpha  \cdot V\left(\frac{\pr}{\alpha}\right)}
\leq \frac{1}{(1-\eps)g}
\end{align*}
That is, we have the desired bound on the value of the output distribution $V(\px) \geq (1-\eps)g \cdot V\left(\po\right)$. Additionally, Lemma~\ref{lem:fair} proves the fairness guarantee, $\TV(\px,\po) \leq \alpha$, on the output distribution of Algorithm~\ref{alg:cap}. The stated claim thereby follows.
\end{proof}

\subsection{Simple Mixing to achieve Fairness and Welfare guarantees}
In this section, we provide another algorithm, which we call $\smix$ that, for any instance of fair-welfare maximization problem with a distance threshold of $\alpha>0$ attains an approximation factor of $\left(\alpha \\
g+(1-\alpha)^2\right)$ with access of $g$-approximation algorithm for maximizing the welfare value function. For a given instance, our algorithm simply returns the output of the $g$-approximation algorithm with probability $\alpha$, and otherwise, outputs a solution drawn from the fair prior $\pf$. Note that, this can be interpreted as an interpolation between the $g$-approximation solution with $\alpha$ mass and the fair prior distribution scaled with a factor of $1-\alpha$. We begin with the formal description of $\smix$ in Algorithm~\ref{alg:2approx} below.

\input{code/epsilon_mix.tex}

\begin{lemma}\label{lem:fairsimple}
Consider an instance  $\mathcal{P}(V,\pf,\alpha)$ of the fair-welfare maximization problem with value function $V$ and fair prior $p^f$. Let $A$ be the output distribution of Algorithm~\ref{alg:2approx} and $\pa_i=\p\left[A=i\right]$ be the probability  that the algorithm chooses index~$i \in \Sol$. Then, we have
\begin{align*}
  \TV(\pa,\pf) = \frac{1}{2}\sum_{i} |\pa_i-\pf_i|\leq \alpha.
 \end{align*}
\end{lemma}


\begin{proof}
To begin with, note that, we can write
\begin{align*}
\pa_i:=\begin{cases}
\alpha  +(1-\alpha )\pf_i \quad \text{ if, }  i=G\\
(1-\alpha )\pf_i \qquad \quad \text{ if, } i\not=G \text{ and } i\in \text{supp}\left(\pf\right)\\
0 \qquad \qquad \qquad \ \ \text{ otherwise. }
\end{cases}
\end{align*}
This implies that $\pa_G\geq \pf_G$ and $\pa_i\leq \pf_i$ for $i\not=G$. Thus we can write
\begin{align*}
&\ \ \ \sum_{i \in \Sol} \left| \pa_i-\pf_i \right|
=\alpha  +\left(1-\alpha \right)
\cdot\pf_{G}-\pf_{G}\\ +& \sum_{i \in \Sol \setminus \{G\}}\pf_i-\left(1-\alpha \right)\pf_i\leq\sum_{i \in \Sol \setminus \{G\}} \alpha\pf_i+\alpha\leq2\alpha
\end{align*}
which completes the proof.
\end{proof}

\begin{theorem} \label{thm:smix}
Consider an instance  $\mathcal{P}(V,\pf,\alpha)$ of the fair-welfare maximization problem with optimal solution $\po$. Then, using a $g$-approximation algorithm for maximizing the welfare function $V$, Algorithm~\ref{alg:2approx} finds a distribution $A$ over the solution space $\Sol$ such that it achieves following fairness and welfare guarantees.
\begin{align*}
\TV(\pa,\pf) &\leq \alpha,  \ \text{and} \\ \  V(\pa)   
&\geq \min\{g,\alpha g+(1-\alpha)^2\} \cdot V(\po)
\end{align*}
\end{theorem}


\begin{proof}
For an instance,  $\mathcal{P}(V,\pf,\alpha)$ of the fair-welfare maximization problem, Algorithm ~\ref{alg:2approx} chooses the output $G$ of the $g$-approximation algorithm with probability $\alpha$, and otherwise, it samples a solution from the fair prior $p^f$. Therefore, we can write the expected value of the output of Algorithm~\ref{alg:2approx} as 
\begin{align} \label{eq:spa}
  V(\pa)=\alpha  \cdot V(G)+(1-\alpha ) \cdot V\left( \pf \right)  
\end{align}
We will split our analysis into two cases depending on the value $V(\pf)$ of the fair prior with respect to the optimal value $V(\po)$. First, if the value $V(\pf)\geq (1-\alpha )V(\ou)$, we have the following desired bound on value $V(\pa)$ achieved by the output distribution.
\begin{align*}
\frac{V\left(\po\right)}{V\left(\pa\right)}&=\frac{V\left(\po\right)}{\alpha  \cdot V(G)+(1-\alpha ) \cdot V\left(\pf\right)} \\
&\leq \frac{1}{\alpha g+(1-\alpha )^2}.
\end{align*}
Therefore, let us assume that $V(\pf)\leq (1-\alpha )V(\ou)$. Recalling the notations described in Theorem~\ref{thm:emix} and following equation~(\ref{eq:po}), we can write the optimal value $V(\po)$ as,
\begin{align} \label{eq:spo}
V(\po)&=\alpha \cdot V(\ou)+\left(1-\alpha \right)\sum_{i \in \Sol}\frac{\pf_i-\pr_i}{1-\alpha } \cdot V(i) \nonumber\\
&\leq \alpha  \cdot V(\ou)+V(\pf) 
\end{align}
Using equations~(\ref{eq:spa}) and (\ref{eq:spo}), we can write the ratio of the optimal value and the value attained by the output distribution as,
\begin{align*}
\frac{V\left(\po\right)}{V\left(\pa\right)}\leq \frac{\alpha \cdot V(\ou)+V(\pf)}{\alpha g \cdot V(\ou)+(1-\alpha )\cdot V(\pf)}
\end{align*}
Next, we will employ algebraic manipulations to obtain the desired bound for the above ratio.
To this end, consider the function $h(x)=\frac{\alpha  \cdot V(\ou)+x}{\alpha g\cdot V(\ou)+(1-\alpha ) x}$, and its derivative $h'(x)$, as follows
\begin{align*}
%h'(x)&=\frac{\alpha g \cdot V(\ou)+(1-\alpha)x-(1-\alpha )\left(\alpha \cdot  V(\ou)+x\right)}{\left(\alpha g \cdot V(\ou)+(1-\alpha)x\right)^2}\\
\frac{\alpha g \cdot  V(\ou)-\alpha (1-\alpha) \cdot V(\ou)}{\left(\alpha g \cdot V(\ou)+(1-\alpha )x\right)^2}
\end{align*}
We conclude that the function $h(\cdot)$ is either a decreasing or an increasing function, depending on the magnitude of $\alpha g$ and $\alpha(1-\alpha)$. If $h(\cdot)$ is decreasing, then $h(x)\leq h(0)= \frac{1}{g}$ for $x\geq0$ while, if $h(\cdot)$ is increasing, then we have
$h(x)\leq h((1-\alpha ) \cdot V(\ou))= \frac{1}{\alpha g+(1-\alpha )^2}$ for $x\leq (1-\alpha) \cdot V(\ou)$. Overall, for the case when $V(\pf)\leq (1-\alpha )V(\ou)$, we obtain
\begin{align*}
\frac{V\left(\po\right)}{V\left(\pa\right)}\leq \max\{\frac{1}{g},\frac{1}{\alpha g+(1-\alpha )^2}\}.
 \end{align*}
Thus, we conclude that this is always the case which implies 
\begin{gather*}
V(\pa)\geq \min\{g,\alpha g+(1-\alpha)^2\} \cdot V(\po).
\end{gather*}
This completes our proof and establishes the stated claim.
\end{proof}
\begin{remark}\label{rmk:tight}
Consider an instance of the fair-welfare maximization problem wherein the fair prior $\pf$ is such that any solution in its support $\text{supp}(\pf)$ has a welfare value of $0$ and $V(G)=g \cdot V(\ou)$. Note that, in this case, using Lemma~\ref{lem:opt}, we have $V(\po)=\alpha \cdot V(\ou)$. Therefore, using equation~(\ref{eq:spa}), we know that the value of the output distribution of $\smix$ must be $V(\pa)=\alpha g \cdot V(\ou)=g  \cdot V(\po)$. Observe that, the factor $g$ in the minimum of the lower bound of $\smix$'s welfare (\cref{thm:smix}), is therefore necessary for $g\leq\alpha g+(1-\alpha)^2$ i.e. $\alpha\leq 1-g$. So we can come up with an instance for arbitrary small $\alpha>0$ where the lower bound being $g$ is necessary for it to be tight. 

Furthermore, note that for such an instance of the fair-welfare maximization problem, the value of the output distribution of $\emix$ is $V(\px)=(1-\eps)\alpha  \cdot V(G)= (1-\eps)\alpha g \cdot V(\ou)= (1-\eps)g \cdot V(\po)$, implying that the lower bound of the welfare for $\emix$ in Theorem~\ref{thm:emix} is tight. Another interesting thing to note here is the above instance, the welfare guarantee of $\smix$ is an additive factor $\eps\alpha g \cdot V(\ou)$ better than that of $\emix$. The case when $\smix$ performs better than $\emix$, in general, would be true whenever the fair prior $\pf$ is such that all the solutions in its support have the same welfare and this welfare is smaller than $V(G)$. This is true since choosing from the top $1-(1-\eps)\alpha$-fraction highest welfare solutions in a sample from $\pf$ ($\emix$) is the same as just choosing one sample from $\pf$ ($\smix)$. Thus the extra $\eps\alpha$ mass that $\smix$ gets to put on the approximate solution gives it a higher expected welfare. 

To reiterate, this behavior generalizes to the case when the solutions in support set $\text{supp}\left(\pf\right)$ do not differ much in terms of their welfare values, i.e. they are in a narrow range, and the welfare of the approximation algorithms is sufficiently larger (depending on $\eps$) than the values in the range. Furthermore, we note that as $\eps$ converges towards zero, $\emix$ obtains just as good guarantees on its welfare as $\smix$. This happens since $V(\px)\geq g\cdot(1-\eps) \cdot V(\po)$ and $V(\pa)\geq \min\{g,\alpha g+(1-\alpha)^2\} \cdot V(\po)$. 

We now present an series of examples of a fair-welfare maximization problem with $g=1$ thus $g>\alpha g+(1-\alpha)^2$, so $\min\{g,\alpha g+(1-\alpha)^2\}=\alpha g+(1-\alpha)^2$, and for a specific $\alpha'$ we have $V(\pa)=(\alpha'g+(1-\alpha')^2)V(\po)$. The $\alpha'$ specifies the examples, and $\alpha'$ can be chosen to be any number between $0$ and $1.$ Thus combined with the above example we have shown that for any $\alpha\leq 1-g$ and for $g=1$ $\alpha \in [0,1]$ there exists fair-welfare maximization problems such that both of the values in the $\min$ in the lower bound for the welfare of $\smix$ is attained with equality, so tight for these values of $g$ and $\alpha$. Now consider the following welfare maximization problem, with 3 solutions $S_1$, $S_2$ and $S_3$, where $V(S_1)=1$, $V(S_2)=1$ and $V(S_3)=0$. Further let the fair prior put $\beta$ mass on  $S_2$ and  $1-\beta$ mass on $S_3$, thus $V(\pf)=\beta$ for $\beta\in[0,1]$. Let the approximation algorithm output $S_1$, thus $g=1$. This implies that $V(\pa)=\alpha+(1-\alpha)\beta$ and $V(\po)=\min\{\beta+\alpha,1\}$. Furthermore we have that $\min\{g,\alpha+(1-\alpha)^2\}=\alpha+(1-\alpha)^2$ since $g=1$. Now for $\alpha'=1-beta$ we get that $V(\pa)=\alpha'+(1-\alpha')^2$, $V(\po)=1$ and $\alpha'+(1-\alpha')^2=$. Since the above holds for any $\beta \in [0,1]$ we can make an example fo any $\alpha\in[0,1]$, i.e. we conclude that the lower bound of $\smix$ is tight. 
%Next, to see that $\emix$ can be better than $\smix$, we consider the following fair-welfare maximization problem. Consider a where $V(S_1)=1$,$V(S_2)=1/2$ and $V(S_3)=0$. Let us assume that the $g$-approximation algorithm outputs $S_1$, implying that $g=1$. Let us further assume that the fair prior puts a mass of $1/2$ on each of $S_2$ and $S_3$, thus $V(\pf)=1/4$. This implies that $V(\px)=\alpha+(1-\alpha) \cdot V(\pf)=\alpha+(1-\alpha)/4$. Further, note that $V(\po)=\alpha+\min\{1-\alpha,1/2\}/2$. Therefore, for $0<\alpha<1$ we have $V(\po)>V(\px)$. Now, using the fact that $V(\pa)\geq (1-\eps)\cdot V(\po)$, we conclude that for any $0<\alpha<1$ there exists an $\eps_\alpha$ such that $V(\pa)>V(\px)$. In total, we conclude that $\emix$ can be strictly better than $\smix$. The following experiments will indicate the above remarks about the performance of $\smix$ compared to $\emix$ for fair-welfare maximization problem. 

\end{remark}


==> sections/oldest_alg.tex <==
\section{Our Algorithm}

\iffalse
Given an instance of fair influence maximization, our algorithm (\textsc{Alg}) begins with solving the problem without the fairness constraint. It does so by running the well-known greedy algorithm that successively picks nodes (to include in the seeding) who maximizes the marginal influence over the graph. Recall that it has $(1-1/e)$-approximation to the unconstrained influence maximization problem. Let us denote the output of the greedy algorithm by $g \in \{0,1\}^n$ with $||g||=k$. With the vector $g$ in hand, we interpolate between $g$ and $t$ in order to find the convex combination $z_\alpha := \alpha \cdot g + (1- \alpha) \cdot t$ of vectors $g$ and $t$ for $\alpha \in [0,1]$ that is at most $D$ away from $t$ with respect to their KL-divergence and maximizes the influence in the graph. Note that $z_\alpha \in [0,1]^n$ and $||z_\alpha|| = k$.
\begin{align*}
\max_{\alpha \in [0,1] } F'(z_\alpha)\\
\text{subject to} \ KL(t,z_\alpha) \leq D \\
\end{align*}


\subsection{Analysis}
Consider an instance of fair influence maximization with $g$ as the output from the greedy algorithm for the unconstrained version. Let us denote $g_1$ to be the first node selected by the greedy algorithm. 
Then, we have
$$ F(g_1) \geq  \frac{1}{k} F(g)$$
% Let us denote the set corresponding to $g$ as $S_k$ of size $k$, and  $g_1$ be the first node chosen by the greedy algorithm. 

Note that we have the following trivial relation about the performance of \textsc{Alg}.

$$ F'(\textsc{Alg}) = F'(z_\alpha) = \alpha \left(1-\frac{1}{e} \right)\textsc{OPT} + (1- \alpha) F'(t)$$
\fi

\subsection{Analysis}


\begin{algorithm}
\caption{Take input $\alpha,\eps$}\label{alg:cap}
\begin{algorithmic}
\Require That $\alpha$ and $\eps$ are rational numbers 
\State Set $s$ to be the smallest integer larger than $(\left(\alpha/2)\eps\right)^{-2}\log\left(K\left(1+\eps\right)/\eps\right)$ which is a multiple of $\alpha/2(1-\eps)$.
\State Run the guaranteed algorithm and let the outcome be $\sg$.
\State Flip a coin with probability $(\alpha/2)(1-\eps)$ for heads.
\If{the coin flip came out heads}
   \State{Return $\sg$}
\Else
   \State{Sample $s$ times from $\pf$ and denote the sample $Z$}
   \State{Mark the $(\alpha/2)(1-\eps)s$ items in $Z$ with the smallest $V(\cdot)$}
   \State{Pick a item between the unmarked items from $Z$ uniformly at random and output that item}
\EndIf
\end{algorithmic}
\end{algorithm}

\begin{lemma}
Fairness constraint
\end{lemma}

\begin{proof}
Consider a random vector $Z_s$ with $s$ entries, where each entry is a index for a item sampled from $\pf$. Let know $Y$ be a random variable independent of $Z_s$ which chooses a number between $1,\ldots,s$. Let $\pz$ be the law of $(Z_s)_{Y}$, since we have that $\pz$ is the same as $\pf$ we may just as well work with $\pz$. 


Now consider the following random mechanism $T(\cdot)$ and random variable $X$.The random mechanism $T(\cdot)$  takes in $s$ indexes and mark the $\beta s$ (where $\beta$ is a number in $[0,1]$ such that $\beta s$ is an integer) which has the smallest $V(\cdot)$-values, if there are indexes with the same value of $V(\cdot)$ it picks one of the indexes and marks as many as its indexes as possible, before continuing to the next. After marking the items after increasing $V(\cdot)$-values starting from the smallest it then uniformly at random pick one of the unmarked items. First the random variable $X$ flips a coin which comes up with heads with probability $\beta$, if the outcome of this coin flip is heads it outputs the index $G$, else X output the random variable $T(Z_s)$. Let now $\px$ be the law of $X$.
Notice that by the law of total probability we have that 
\begin{align*}
\px_{i}=\p\left[X=i\right]=\mathbbm{1}_{G=i}\beta+\p\left[T(Z_s)=i\right]\left(1-\beta\right)
\end{align*}

Using this we get that

\begin{align*}
&\sum_{i} |\px_i-\pz_i|\\
&=\sum_{i} |\p\left[X=i\right]-\p\left[(Z_s)_{Y}=i\right]|\\
&=\sum_{i} |\mathbbm{1}_{G=i}\beta+\p\left[T(Z_s)=i\right]\left(1-\beta\right)-\p\left[(Z_s)_{Y}=i\right]|\\
&=\sum_{i} |\sum_{z_s\in (\text{supp}(\pf))^s} \left(\mathbbm{1}_{G=i}\beta+\p\left[T(z_s)=i\right](1-\beta)-\p\left[(z_s)_{Y}=i\right]\right)\p(Z_s=z_s)|\\
&\leq \sum_{z_s\in (\text{supp}(\pf))^s} \p(Z_s=z_s) \left(\sum_{i} | \left(\mathbbm{1}_{G=i}\beta+\p\left[T(z_s)=i\right](1-\beta)-\p\left[(z_s)_{Y}=i\right]\right)|\right).
\end{align*}

Where the last equality follows by the law of total expectation and the inequality by repeated use of the triangle inequality. Thus if we can bound $\sum_{i} | \left(\mathbbm{1}_{G=i}\beta+\p\left[T(z_s)=i\right](1-\beta)-\p\left[(z_s)_{Y}=i\right]\right)|$ with something less than $\alpha$ for any $z_s\in (\text{supp}(\pf))^s$ we have by the above shown that the total variational distance between $\pz$ and $\pf$ is less than $\alpha$ and we are done. To do this we introduce the following notations. For an $z_s\in (\text{supp}(\pf))^s$ and a index $i$ for an item, we let $(z_s)_i$ denote the number of items with the index $i$ in the $z_s$. We further let $z_s^m$ denote the sample after $T$ have marked $\beta s$ of the items in $z_s$ with the smallest value of $V(\cdot)$ and let  $(z_s^m)_i$ denote the number of items with the index i and not being marked in $z_s^m$. For an $z_s$ we further define the index $i_{0\leq }$ to be the index $i$ which is the index of the marked item with the largest $V(\cdot)$. We notice that if there exist another index $i$ which items are marked and $i$ is not $i_{0\leq }$ then $(z_s^m)_i=0$ since $T$ continued marking items of one index until there where no more items of that index left or it had marked $\beta s$ items and since it did the marking in a increasing order based on the values of $V(\cdot)$ starting from the smallest value and $i_{0\leq }$ is the index of the item in $z_s$ which is marked and has the largest $V(\cdot)$-value of the marked items, it follows that all items with index $i$ must have been marked and hence $(z_s^m)_i=0$. With this notation we notice that since $(z_s)_Y$ is a uniform random sample from the item in $z_s$ we have that for and index $i$ that $\p\left[(z_s)_{Y}=i\right]=(z_s)_{i}/s$, and since $T(z_s)$ is a uniform random sample between the unmarked items (there are $(1-\beta)s$ unmarked items) we get that $\p\left[T(z_s)=i\right]=(z_s^m)_{i}/((1-\beta)s)$.  Thus for an $z_s\in \text{supp}(\pf)^s$ we get that

\begin{align*}
&\sum_{i} | \left(\mathbbm{1}_{G=i}\beta+\p\left[T(z_s)=i\right](1-\beta)-\p\left[(z_s)_{Y}=i\right]\right)|\\
&=\sum_{i} | \mathbbm{1}_{G=i}\beta+\left((z_s^m)_{i}-(z_s)_{i}\right)/s|\\
&=|\beta+\left((z_s^m)_{G}-(z_s)_{G}\right)/s|+\sum_{i: \ 
 i\not = G \text{ and $i$ not marked}} |(\left(z_s^m)_{i}-(z_s)_{i}\right)/s|\\
 &+\mathbbm{1}_{i_{0\leq}\not=G}|\left((z_s^m)_{i_{0\leq}}-(z_s)_{i_{0\leq}}\right)/s|+\sum_{i: \ 
 i\not = G,i_{0\leq} \text{ and $i$ is marked}} |\left((z_s^m)_{i}-(z_s)_{i}\right)/s|\\
 &=\beta+\left((z_s^m)_{G}-(z_s)_{G}\right)/s
 -\mathbbm{1}_{i_{0\leq}\not=G}\left((z_s^m)_{i_{0\leq}}-(z_s)_{i_{0\leq}}\right)/s+\sum_{i: \ 
 i\not = G,i_{0\leq} \text{ and $i$ is marked}} (z_s)_{i}/s\\
\end{align*}
where the last equality follows by $(z_s^m)_{i}=(z_s)_{i}$ for indexes $i$ which doesnt have marked items implying that $\sum_{i: \ 
 i\not = G \text{ and $i$ not marked}} |\left((z_s^m)_{i}-(z_s)_{i}\right)/s|=0$ and that since we marked $\beta s$ items we know that $(z_s^m)_{i}-(z_s)_{i}\geq -\beta s$ which implies that $|\beta+\left((z_s^m)_{G}-(z_s)_{G}\right)/s|=\beta+\left((z_s^m)_{G}-(z_s)_{G}\right)/s$. Now noticing that $\sum_{i: \ 
 i\not = G,i_{0\leq} \text{ and $i$ is marked}} (z_s)_{i}$ is the number of marked items with indexes not equal to $G$ and $i_{0\leq}$. Thus if there is no indexes other than $i_{0\leq}$ and $G$ which are marked the sum is $0$. If there is more indexes than $i_{0\leq}$ and $G$ which items are marked and: 1) $i_{0\leq}\not=G$ we get that the sum is $\beta s-((z_s)_{G}-(z_s^m)_{G})-\left((z_s)_{i_{0\leq}}-(z_s^m)_{i_{0\leq}}\right)$ or 2) if $i_{0\leq}=G$ the sum is $\beta s-((z_s)_{G}-(z_s^m)_{G})$. Hence if no other indexes than $i_{0\leq}$ and $G$ are marked we get that 

\begin{align*}
&\beta+\left((z_s^m)_{G}-(z_s)_{G}\right)/s
 -\mathbbm{1}_{i_{0\leq}\not=G}\left((z_s^m)_{i_{0\leq}}-(z_s)_{i_{0\leq}}\right)/s+\sum_{i: \ 
 i\not = G,i_{0\leq} \text{ and $i$ is marked}} (z_s)_{i}/s\\
 &=\beta+\left((z_s^m)_{G}-(z_s)_{G}\right)/s
 -\mathbbm{1}_{i_{0\leq}\not=G}\left((z_s^m)_{i_{0\leq}}-(z_s)_{i_{0\leq}}\right)/s
 \leq 2\beta
\end{align*}
since as noticed earlier $(z_s^m)_{i}-(z_s)_{i}\geq-\beta s$ and $\left((z_s^m)_{G}-(z_s)_{G}\right)/s$ is non positive. Further if their are other indexes than $i_{0\leq}$ and $G$ which are marked and 1) $i_{0\leq}\not=G$ we get that

\begin{align*}
&\beta+\left((z_s^m)_{G}-(z_s)_{G}\right)/s
 -\mathbbm{1}_{i_{0\leq}\not=G}\left((z_s^m)_{i_{0\leq}}-(z_s)_{i_{0\leq}}\right)/s+\sum_{i: \ 
 i\not = G,i_{0\leq} \text{ and $i$ is marked}} (z_s)_{i}/s\\
 &=\beta+\left((z_s^m)_{G}-(z_s)_{G}\right)/s-
 \left((z_s^m)_{i_{0\leq}}-(z_s)_{i_{0\leq}}\right)/s+\left(\beta s-((z_s)_{G}-(z_s^m)_{G})-\left((z_s)_{i_{0\leq}}-(z_s^m)_{i_{0\leq}}\right)
\right)/s
\leq 2\beta
\end{align*}
since $\left((z_s^m)_{G}-(z_s)_{G}\right)/s$ is non positive, or if 2) $i_{0\leq}=G$ we get that
\begin{align*}
&\beta+\left((z_s^m)_{G}-(z_s)_{G}\right)/s
 -\mathbbm{1}_{i_{0\leq}\not=G}\left((z_s^m)_{i_{0\leq}}-(z_s)_{i_{0\leq}}\right)/s+\sum_{i: \ 
 i\not = G,i_{0\leq} \text{ and $i$ is marked}} (z_s)_{i}/s\\
 &=\beta+\left((z_s^m)_{G}-(z_s)_{G}\right)/s+\left(\beta s-((z_s)_{G}-(z_s^m)_{G})
\right)/s
\leq 2\beta,
\end{align*}
again since $\left((z_s^m)_{G}-(z_s)_{G}\right)/s$ is non positive. Where by we conclude that for any $z_s\in \text{ supp}(Z_s)$ we have that $\sum_{i} | \left(\mathbbm{1}_{G=i}\beta+\p\left[T(z_s)=i\right](1-\beta)-\p\left[(z_s)_{Y}=i\right]\right)|\leq 2\beta$ which as notice earlier implies that 

\begin{align*}
&\sum_{i} |\px_i-\pz_i|\leq \sum_{z_s\in (\text{supp}(\pf))^s} \p(Z_s=z_s) \left(\sum_{i} | \left(\mathbbm{1}_{G=i}\beta+\p\left[T(z_s)=i\right](1-\beta)-\p\left[(z_s)_{Y}=i\right]\right)|\right)
\leq 2\beta,
\end{align*}
which yields the claim of the lemma.
\end{proof}
\begin{lemma}
Approximation guarantee
\end{lemma}

\begin{proof}
Let in the following $\ou$ be the index of optimal item in the unconstrained problem and $G$ be the solution by the approximation algorithm. 

A optimal solution to the constraint problem $\po$ could be constructed in the following manner. Start with $\pf$ and move $\alpha/2$ mass from the indexes of $\pf$ to the index $\ou$ starting with index of smallest $V(\cdot)$ and then in increasing order, we do such that if there is a tie in the $V(\cdot)$ value we choose one of the indexes an move a much mass from this index before continuing to one of the other indexes. In this manner we obtain a solution $\po$ which fullfilles the constraint of being $\alpha$ close to $\pf$ and at the same time putting as much mass onto the index which maximizes $V(\cdot)$ yielding that it is a optimal solution. In the following let $\pr_i$ be the amount of mass moved from the indexes with the smallest $V(\cdot)$ values to the optimal index from the unconstrained problem $\ou$. Notice that $||\pr_i||_1=\alpha/2$, so $||\pr_i||_1/(\alpha/2)$ is a probability distribution. By the above construction of $\po$ we get that
\begin{align}\label{poeq}
 &V\left(\po\right)=\sum_{i}\po_iV(i)=(\alpha/2)V(\ou)+\sum_{i}(\pf_i-\pr_i)V(i)\nonumber\\
 &=(\alpha/2)V\left(\ou\right)+V\left(\pf\right)-(\alpha/2)V\left(\pr/(\alpha/2)\right).
 \end{align}
We now consider $\px$ then we have that
\begin{align*}
 &V\left(\px\right)=\beta V \left(G\right) +\e\left[V\left(T(Z_s)\right)\right](1-\beta)
\end{align*}
Now for a sample $z_s$ in $\text{supp}(\pf)^s$ we have that since $T(z_s)$ is a uniformly random pick between the $(1-\beta)s$ no marked indexes in $z_s$ which is the largest indexes we get that 
\begin{align*}
&\e\left[V\left(T(z_s)\right)\right](1-\beta)\\
&=\sum_{i\in z_s: i \text{ is not marked}} V(i)/s\\
&=\sum_{i\in z_s} V(i)/s-\sum_{i\in z_s:\text{ such that } i \text{ is  marked}} V(i)/s\\
&=\sum_{i=1}^s V({z_s}_i)/s-\sum_{i\in z_s:\text{ such that } i \text{ is  marked}} V(i)/s
 \end{align*}
implying that 
\begin{align*}
&\e\left[V\left(T(Z_s)\right)\right](1-\beta) \\
&=\sum_{i=1}^s \e\left[V({Z_s}_i)\right]/s-\e\left[\sum_{i\in Z_s:\text{ such that } i \text{ is  marked}} V(i)/s\right]\\
&=V(\pf)-\beta \e\left[\sum_{i\in Z_s:\text{ such that } i \text{ is  marked}} V(i)/(\beta s)\right]
\end{align*}
where the last equality follows by the entries of $Z_s$ are independent samples from $\pf$. Where by we conclude that $V(\px)$ is 
\begin{align*}
V(\px)=\beta V \left(G\right) +V(\pf)-\beta \e\left[\sum_{i\in Z_s:\text{ such that } i \text{ is  marked}} V(i)/(\beta s)\right]
\end{align*}
We now want to argue that for $\beta=(\alpha/2)(1-\eps)$ the ratio of $V(\po)/V(\px)$ is not to large. To do this we want to lower bound $V(\px)$ with something close to $V(\po)$. Looking at the expression for $V\left(\po\right)$ in \Cref{poeq} we see that a first step in lower bounding $V(\px)$ could be using he $(1-g)$ approximation guarantee that $G$ has compared to $\ou$ which yields that 
\begin{align}\label{eqalgvaluelowerbound}
V(\px)\geq \beta (1-g)V \left(\ou\right) +V(\pf)-\beta \e\left[\sum_{i\in Z_s:\text{ such that } i \text{ is  marked}} V(i)/(\beta s)\right]
\end{align}
Now looking at the expression for $V\left(\po\right)$ in \Cref{poeq} we see that we dont want to do anything about the $V\left(\pf\right)$-term in $V\left(\px\right)$, and we will focus on the last term. Now we want the term $\e\left[\sum_{i\in Z_s:\text{ such that } i \text{ is  marked}} V(i)/(\beta s)\right]$ to be close to $V\left(\pr/(\alpha/2)\right)$, 
so that the $V(\cdot)$ normalized values of the marked indexes (which are the indexes in $Z_s$ with the smallest $V(\cdot)$-values) in expectation is close to a the expected value of a random variables $V(\cdot)$-value drawn from $\pr/(\alpha/2)$. 

To see that this is the case we image the sampling producer of each item of $Z_s$ in the following manner.  First we flip a coin which comes up heads with probability $\alpha/2$. If the coin flip becomes heads we sample from $\pr/(\alpha/2)$ else we sample from $(\pf-\pr)/(1-\alpha/2)$. Now denote this coins $C_1,\ldots,C_s$ and let $C=\sum_{i=1}^sC_i$ where $C_i$ is $1$ if it comes up heads and $0$ else, hence $C$ 
is counting the amount of heads in the $s$ samples - the number of times we sample from $\pr/(\alpha/2)$. Now since we have that $\e\left[C\right]=(\alpha/2)s$ and $0\leq C_i\leq 1$ we get by Hoeffdings inequality that 
\begin{align*}
\p\left[C-\e\left[C\right]\leq -((\alpha/2)/\eps)s\right]\leq \exp\left(-2s\eps^2 \right)
\end{align*}
Implying that with at probability at least $1-\exp\left(-2s\eps^2 \right)$ the sample $Z_s$ contain more than $E[C]-((\alpha/2)/\eps)s=(\alpha/2)(1-\eps)s=\beta s$ samples from the $\pr/(\alpha/2)$-distribution. Now consider an outcome of $C=c$ such that $c\geq(\alpha/2)(1-\eps)s=\beta s$ and let ${Z_r}_1,\ldots,{Z_r}_c$ be the independent samples from $\pr/(\alpha/2)$ and ${Z_r}^{(1)},\ldots,{Z_r}^{(\beta s)}$ the $\beta s$ first order variables of ${Z_r}_1,\ldots,{Z_r}_c$ we the have that for any permutation $\pi :[\beta s]\rightarrow [c]$ which is injective that
\begin{align*}
 \sum_{i=1}^{\beta s} {Z_{r}}_{\pi(i)}\geq \sum_{i=1}^{\beta s} {Z_{r}}^{(i)} 
 \end{align*}
implying that
\begin{align}\label{ordereq}
 \beta sV(\pr/(\alpha/2))=\e\left[\sum_{i=1}^{\beta s}  {Z_{r}}_{\pi(i)}\right]\geq \e\left[\sum_{i=1}^{\beta s} {Z_{r}}^{(i)} \right] \nonumber\\
V(\pr/(\alpha/2))\geq \e\left[\sum_{i=1}^{\beta s} {Z_{r}}^{(i)} /(\beta s)\right]
 \end{align}
where we have used in the equality that the permutation is deterministic and injective so that the $Z_{\pi(i)}$'s are independent random variables drawn from $\pr/(\alpha/2)$. 

Now looking back at $\e\left[\sum_{i\in Z_s:\text{ such that } i \text{ is  marked}} V(i)/(\beta s)\right]$ we see that $\sum_{i\in Z_s:\text{ such that } i \text{ is  marked}} V(i)/(\beta s)=\sum_{i=1}^{\beta s} Z^{(i)}/(\beta s)$, where the order variables $Z^{(i)}$ first order the ${Z_{r}}_j$ in the sample and then remaining elements not picked by $\pr/(\alpha/2)$, which we can do since we know that ${Z_r}_{i}\leq {Z_\slashed{r}}_{j}$, for any $i,j$ where ${Z_\slashed{r}}_{j}$ is a index in the sampled picked by $(\pf-\pr)/((1-\beta)s)$. Now for outcomes of $C=c\geq  \beta s$ we then have that $Z_s$ contain ${Z_r}_{1},\ldots,{Z_r}_{c}$ independent samples from $\pr/(\alpha/2)$, which implies that $\sum_{i\in Z_s:\text{ such that } i \text{ is  marked}} V(i)/(\beta s)=\sum_{i=1}^{\beta s} {Z_r}^{(i)}/(\beta s)$, and thus by \Cref{ordereq} we get that for such outcomes of $c\geq \beta s$ of $C$ we get that 
\begin{align*}
\e\left[\sum_{i\in Z_s:\text{ such that } i \text{ is  marked}} V(i)/(\beta s)\mid C\geq \beta s\right]=\sum_{i=1}^{\beta s} \e\left[{Z_r}^{(i)}/(\beta s)\right]\leq V(\pr/(\alpha/2)).
\end{align*}
Thus using the law of total expectation and that $V(\cdot)$ is bounded by $K$ from above, and $1$ from below we get by using an sample size $s\geq (\left(\alpha/2)\eps\right)^{-2}\log\left(K\left(1+\eps\right)/\eps\right)=((\alpha/2)/\eps)^{-2}\log\left(K\beta/((\alpha/2)/\eps)\right)$ that 
\begin{align*}
\e\left[\sum_{i\in Z_s:\text{ such that } i \text{ is  marked}} V(i)/(\beta s)\right] &\leq V(\pr/(\alpha/2))(1-\exp\left(-s((\alpha/2)/\eps)^2)\right)+\exp(-s((\alpha/2)/\eps)^2)K\\
&\leq V(\pr/(\alpha/2))+K\exp(-s((\alpha/2)/\eps)^2)
= V(\pr/(\alpha/2))(1+((\alpha/2)/\eps)/\beta)
\end{align*}
Now plugging this back into \Cref{eqalgvaluelowerbound} and using that $\beta=(\alpha/2)(1-\eps)$ we obtain that
\begin{align}\label{lowerpx}
V(\px)&\geq \beta (1-g)V \left(\ou\right) +V(\pf)-\beta(1+((\alpha/2)/\eps)/\beta) V(\pr/(\alpha/2))\nonumber\\
&=\beta (1-g)V \left(\ou\right) +V(\pf)-(\beta+((\alpha/2)/\eps)) V(\pr/(\alpha/2))\\
&=\beta (1-g)V \left(\ou\right) +V(\pf)-(\alpha/2) V(\pr/(\alpha/2))\nonumber.
\end{align}
Now using that for $a>b$ and $x>0$ we have that $(a+x)/(b+x)\leq a/b$, with $a=(\alpha/2)V \left(\ou\right) $, $b=\beta (1-g)V \left(\ou\right) $ and $x=V(\pf)-(\alpha/2) V(\pr/(\alpha/2))$, together with \Cref{poeq} and \Cref{lowerpx} we get that
\begin{align*}
\frac{V\left(\po\right)}{V(\px)}
\leq \frac{(\alpha/2)V\left(\ou\right)+V\left(\pf\right)-(\alpha/2)V\left(\pr/(\alpha/2)\right)}{\beta (1-g)V \left(\ou\right) +V(\pf)-(\alpha/2) V(\pr/(\alpha/2))}
\leq \frac{1}{(1-\eps)(1-g)}
\end{align*}
implying that $(1-\eps)(1-g)V\left(\po\right)\leq V(\px)$ with $s=\left\lceil(\left(\alpha/2)\eps\right)^{-2}\log\left(K\left(1+\eps\right)/\eps\right)\right\rceil$ many samples.


\end{proof}




==> sections/oldremark.tex <==


We will now make the following remarks on $\emix$ and $\smix$.
\begin{enumerate}
    \item $V(\px)\geq V(\pa)$ that is the expected welfare of $\emix$ is always greater than $\smix$
\end{enumerate}
Consider an instance of the fair-welfare maximization problem wherein the fair prior $\pf$ is such that any solution in its support $\text{supp}(\pf)$ has a welfare value of $0$ and $V(G)=g \cdot V(\ou)$. Note that, in this case, using Lemma~\ref{lem:opt}, we have $V(\po)=\alpha \cdot V(\ou)$. Therefore, using equation~(\ref{eq:spa}), we know that the value of the output distribution of $\smix$ must be $V(\pa)=\alpha g \cdot V(\ou)=g  \cdot V(\po)$. Observe that, the factor $g$ in the minimum of the lower bound of $\smix$'s welfare (\cref{thm:smix}), is therefore necessary for $g\leq\alpha g+(1-\alpha)^2$ i.e. $\alpha\leq 1-g$. So we can come up with an instance for arbitrary small $\alpha>0$ where the lower bound being $g$ is necessary for it to be tight. 

Furthermore, note that for such an instance of the fair-welfare maximization problem, the value of the output distribution of $\emix$ is $V(\px)=(1-\eps)\alpha  \cdot V(G)= (1-\eps)\alpha g \cdot V(\ou)= (1-\eps)g \cdot V(\po)$, implying that the lower bound of the welfare for $\emix$ in Theorem~\ref{thm:emix} is tight. Another interesting thing to note here is the above instance, the welfare guarantee of $\smix$ is an additive factor $\eps\alpha g \cdot V(\ou)$ better than that of $\emix$. The case when $\smix$ performs better than $\emix$, in general, would be true whenever the fair prior $\pf$ is such that all the solutions in its support have the same welfare and this welfare is smaller than $V(G)$. This is true since choosing from the top $1-(1-\eps)\alpha$-fraction highest welfare solutions in a sample from $\pf$ ($\emix$) is the same as just choosing one sample from $\pf$ ($\smix)$. Thus the extra $\eps\alpha$ mass that $\smix$ gets to put on the approximate solution gives it a higher expected welfare. 

To reiterate, this behavior generalizes to the case when the solutions in support set $\text{supp}\left(\pf\right)$ do not differ much in terms of their welfare values, i.e. they are in a narrow range, and the welfare of the approximation algorithms is sufficiently larger (depending on $\eps$) than the values in the range. Furthermore, we note that as $\eps$ converges towards zero, $\emix$ obtains just as good guarantees on its welfare as $\smix$. This happens since $V(\px)\geq g\cdot(1-\eps) \cdot V(\po)$ and $V(\pa)\geq \min\{g,\alpha g+(1-\alpha)^2\} \cdot V(\po)$. 

We now present an series of examples of a fair-welfare maximization problem with $g=1$ thus $g>\alpha g+(1-\alpha)^2$, so $\min\{g,\alpha g+(1-\alpha)^2\}=\alpha g+(1-\alpha)^2$, and for a specific $\alpha'$ we have $V(\pa)=(\alpha'g+(1-\alpha')^2)V(\po)$. The $\alpha'$ specifies the examples, and $\alpha'$ can be chosen to be any number between $0$ and $1.$ Thus combined with the above example we have shown that for any $\alpha\leq 1-g$ and for $g=1$ $\alpha \in [0,1]$ there exists fair-welfare maximization problems such that both of the values in the $\min$ in the lower bound for the welfare of $\smix$ is attained with equality, so tight for these values of $g$ and $\alpha$. Now consider the following welfare maximization problem, with 3 solutions $S_1$, $S_2$ and $S_3$, where $V(S_1)=1$, $V(S_2)=1$ and $V(S_3)=0$. Further let the fair prior put $\beta$ mass on  $S_2$ and  $1-\beta$ mass on $S_3$, thus $V(\pf)=\beta$ for $\beta\in[0,1]$. Let the approximation algorithm output $S_1$, thus $g=1$. This implies that $V(\pa)=\alpha+(1-\alpha)\beta$ and $V(\po)=\min\{\beta+\alpha,1\}$. Furthermore we have that $\min\{g,\alpha+(1-\alpha)^2\}=\alpha+(1-\alpha)^2$ since $g=1$. Now for $\alpha'=1-beta$ we get that $V(\pa)=\alpha'+(1-\alpha')^2$, $V(\po)=1$ and $\alpha'+(1-\alpha')^2=$. Since the above holds for any $\beta \in [0,1]$ we can make an example fo any $\alpha\in[0,1]$, i.e. we conclude that the lower bound of $\smix$ is tight. 
%Next, to see that $\emix$ can be better than $\smix$, we consider the following fair-welfare maximization problem. Consider a where $V(S_1)=1$,$V(S_2)=1/2$ and $V(S_3)=0$. Let us assume that the $g$-approximation algorithm outputs $S_1$, implying that $g=1$. Let us further assume that the fair prior puts a mass of $1/2$ on each of $S_2$ and $S_3$, thus $V(\pf)=1/4$. This implies that $V(\px)=\alpha+(1-\alpha) \cdot V(\pf)=\alpha+(1-\alpha)/4$. Further, note that $V(\po)=\alpha+\min\{1-\alpha,1/2\}/2$. Therefore, for $0<\alpha<1$ we have $V(\po)>V(\px)$. Now, using the fact that $V(\pa)\geq (1-\eps)\cdot V(\po)$, we conclude that for any $0<\alpha<1$ there exists an $\eps_\alpha$ such that $V(\pa)>V(\px)$. In total, we conclude that $\emix$ can be strictly better than $\smix$. The following experiments will indicate the above remarks about the performance of $\smix$ compared to $\emix$ for fair-welfare maximization problem. 



==> sections/oldsimple.tex <==
\subsection{Simple Mixing to achieve Fairness and Welfare guarantees}
In this section, we provide another algorithm, which we call $\smix$ that, for any instance of fair-welfare maximization problem with a distance threshold of $\alpha>0$ attains an approximation factor of $\left(\alpha \\
g+(1-\alpha)^2\right)$ with access of $g$-approximation algorithm for maximizing the welfare value function. For a given instance, our algorithm simply returns the output of the $g$-approximation algorithm with probability $\alpha$, and otherwise, outputs a solution drawn from the fair prior $\pf$. Note that, this can be interpreted as an interpolation between the $g$-approximation solution with $\alpha$ mass and the fair prior distribution scaled with a factor of $1-\alpha$. We begin with the formal description of $\smix$ in Algorithm~\ref{alg:2approx} below.

\input{code/epsilon_mix.tex}

\begin{lemma}\label{lem:fairsimple}
Consider an instance  $\mathcal{P}(V,\pf,\alpha)$ of the fair-welfare maximization problem with value function $V$ and fair prior $p^f$. Let $A$ be the output distribution of Algorithm~\ref{alg:2approx} and $\pa_i=\p\left[A=i\right]$ be the probability  that the algorithm chooses index~$i \in \Sol$. Then, we have
\begin{align*}
  \TV(\pa,\pf) = \frac{1}{2}\sum_{i} |\pa_i-\pf_i|\leq \alpha.
 \end{align*}
\end{lemma}


\begin{proof}
To begin with, note that, we can write
\begin{align*}
\pa_i:=\begin{cases}
\alpha  +(1-\alpha )\pf_i \quad \text{ if, }  i=G\\
(1-\alpha )\pf_i \qquad \quad \text{ if, } i\not=G \text{ and } i\in \text{supp}\left(\pf\right)\\
0 \qquad \qquad \qquad \ \ \text{ otherwise. }
\end{cases}
\end{align*}
This implies that $\pa_G\geq \pf_G$ and $\pa_i\leq \pf_i$ for $i\not=G$. Thus we can write
\begin{align*}
&\ \ \ \sum_{i \in \Sol} \left| \pa_i-\pf_i \right|
=\alpha  +\left(1-\alpha \right)
\cdot\pf_{G}-\pf_{G}\\ +& \sum_{i \in \Sol \setminus \{G\}}\pf_i-\left(1-\alpha \right)\pf_i\leq\sum_{i \in \Sol \setminus \{G\}} \alpha\pf_i+\alpha\leq2\alpha
\end{align*}
which completes the proof.
\end{proof}

\begin{theorem} \label{thm:smix}
Consider an instance  $\mathcal{P}(V,\pf,\alpha)$ of the fair-welfare maximization problem with optimal solution $\po$. Then, using a $g$-approximation algorithm for maximizing the welfare function $V$, Algorithm~\ref{alg:2approx} finds a distribution $A$ over the solution space $\Sol$ such that it achieves following fairness and welfare guarantees.
\begin{align*}
\TV(\pa,\pf) &\leq \alpha,  \ \text{and} \\ \  V(\pa)   
&\geq \min\{g,\alpha g+(1-\alpha)^2\} \cdot V(\po)
\end{align*}
\end{theorem}


\begin{proof}
For an instance,  $\mathcal{P}(V,\pf,\alpha)$ of the fair-welfare maximization problem, Algorithm ~\ref{alg:2approx} chooses the output $G$ of the $g$-approximation algorithm with probability $\alpha$, and otherwise, it samples a solution from the fair prior $p^f$. Therefore, we can write the expected value of the output of Algorithm~\ref{alg:2approx} as 
\begin{align} \label{eq:spa}
  V(\pa)=\alpha  \cdot V(G)+(1-\alpha ) \cdot V\left( \pf \right)  
\end{align}
We will split our analysis into two cases depending on the value $V(\pf)$ of the fair prior with respect to the optimal value $V(\po)$. First, if the value $V(\pf)\geq (1-\alpha )V(\ou)$, we have the following desired bound on value $V(\pa)$ achieved by the output distribution.
\begin{align*}
\frac{V\left(\po\right)}{V\left(\pa\right)}&=\frac{V\left(\po\right)}{\alpha  \cdot V(G)+(1-\alpha ) \cdot V\left(\pf\right)} \\
&\leq \frac{1}{\alpha g+(1-\alpha )^2}.
\end{align*}
Therefore, let us assume that $V(\pf)\leq (1-\alpha )V(\ou)$. Recalling the notations described in Theorem~\ref{thm:emix} and following equation~(\ref{eq:po}), we can write the optimal value $V(\po)$ as,
\begin{align} \label{eq:spo}
V(\po)&=\alpha \cdot V(\ou)+\left(1-\alpha \right)\sum_{i \in \Sol}\frac{\pf_i-\pr_i}{1-\alpha } \cdot V(i) \nonumber\\
&\leq \alpha  \cdot V(\ou)+V(\pf) 
\end{align}
Using equations~(\ref{eq:spa}) and (\ref{eq:spo}), we can write the ratio of the optimal value and the value attained by the output distribution as,
\begin{align*}
\frac{V\left(\po\right)}{V\left(\pa\right)}\leq \frac{\alpha \cdot V(\ou)+V(\pf)}{\alpha g \cdot V(\ou)+(1-\alpha )\cdot V(\pf)}
\end{align*}
Next, we will employ algebraic manipulations to obtain the desired bound for the above ratio.
To this end, consider the function $h(x)=\frac{\alpha  \cdot V(\ou)+x}{\alpha g\cdot V(\ou)+(1-\alpha ) x}$, and its derivative $h'(x)$, as follows
\begin{align*}
%h'(x)&=\frac{\alpha g \cdot V(\ou)+(1-\alpha)x-(1-\alpha )\left(\alpha \cdot  V(\ou)+x\right)}{\left(\alpha g \cdot V(\ou)+(1-\alpha)x\right)^2}\\
\frac{\alpha g \cdot  V(\ou)-\alpha (1-\alpha) \cdot V(\ou)}{\left(\alpha g \cdot V(\ou)+(1-\alpha )x\right)^2}
\end{align*}
We conclude that the function $h(\cdot)$ is either a decreasing or an increasing function, depending on the magnitude of $\alpha g$ and $\alpha(1-\alpha)$. If $h(\cdot)$ is decreasing, then $h(x)\leq h(0)= \frac{1}{g}$ for $x\geq0$ while, if $h(\cdot)$ is increasing, then we have
$h(x)\leq h((1-\alpha ) \cdot V(\ou))= \frac{1}{\alpha g+(1-\alpha )^2}$ for $x\leq (1-\alpha) \cdot V(\ou)$. Overall, for the case when $V(\pf)\leq (1-\alpha )V(\ou)$, we obtain
\begin{align*}
\frac{V\left(\po\right)}{V\left(\pa\right)}\leq \max\{\frac{1}{g},\frac{1}{\alpha g+(1-\alpha )^2}\}.
 \end{align*}
Thus, we conclude that this is always the case which implies 
\begin{gather*}
V(\pa)\geq \min\{g,\alpha g+(1-\alpha)^2\} \cdot V(\po).
\end{gather*}
This completes our proof and establishes the stated claim.
\end{proof}
